The regularity problem with a weaker condition on only the transversal direction

We study an elliptic operator $L:=\mathrm{div}(A\nabla \cdot)$ on the upper half space. It is known that if the matrix $A$ is independent in the transversal $t$-direction, then the regularity boundary value problem is solvable with data in a Sobolev space. In the present paper we improve on the $t$-independence condition by introducing a mixed $L^1-L^\infty$ condition that only depends on $\partial_t A$, the derivative of $A$ in transversal direction. This condition is different from other conditions in the literature and has already been proven to imply solvability of the Dirichlet boundary value problem.

==> HeatSemigroup.tex <==
\section{Kato conjecture and properties of the heat semigroup}

In this section we assume to have a uniform elliptic \(t\)-independent operator \(L\), i.e. \(Lu(x)=\Div_x(\AP(x)\nabla u(x))\) for \(x\in\mathbb{R}^n\). In particular, these results apply to the family of operators \(L^s\).
\smallskip

The first result was previously known as the Kato conjecture for \(p=2\), and can be found as Theorem 4.77 in \cite{hofmann_lp_2022}. Note that we define \(\dot W^{1,p}(\mathbb{R}^n)\) as the closure of \(C_0^\infty(\mathbb{R}^n)\) under the seminorm given by \(\Vert f\Vert_{\dot W^{1,p}}:=\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\).
\begin{prop}\label{prop:KatoConjecture}
    For a function \(f\in \dot W^{1,p}(\mathbb{R}^n)\) we have
    \[\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\]
    for all \(1<p<\infty\). Furthermore, there exists \(\varepsilon_1>0\) such that if \(1<p<2+\varepsilon_1\) then
    \[\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}.\]
\end{prop}

A direct consequence is the following corollary 
\begin{cor}\label{cor:NablaL^-1/2Bounded}
    For a function \(f\in L^2(\mathbb{R}^n)\) we have
    \[\Vert \nabla L^{-1/2} f\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}\]
    and if f is a vector valued function
    \[\Vert L^{-1/2} \Div(f)\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}.\]
\end{cor}



\begin{prop}[Proposition 4.3  from \cite{hofmann_dirichlet_2022}]\label{prop:L2NormBoundsOfHeatSemigroup}
If \(L\) is t-independent then the following norm estimates hold for \(f\in L^2(\mathbb{R}^n),l\in \mathbb{N}_0, t>0\) and constants \(c_l,C>0\):

\begin{itemize}
    \item \(\Vert \partial_t^l e^{-tL}f\Vert_{L^2(\mathbb{R}^n)}\leq c_l t^{-l} \Vert f\Vert_{L^2(\mathbb{R}^n)}\),
    \item \(\Vert \nabla e^{-tL}f\Vert_{L^2(\mathbb{R}^n)}\leq C t^{-1/2} \Vert f\Vert_{L^2(\mathbb{R}^n)}\).
\end{itemize}
\end{prop}

The following proposition is a generalization of Equation (5.6) in \cite{hofmann_lp_2022} and its proof also borrows the main ideas from there.

\begin{prop}\label{prop:L2NormGoesTo0}
If we have a compact set \(K\subset\mathbb{R}^n\), a family \(f_s\in W_0^{1,2}(K)\) and a family of uniform elliptic operators \(L^s\) with the same constants \(\lambda_0\) and \(\Lambda_0\) then
\[\lim_{s\to \infty}\Vert e^{-sL^s}f_s\Vert_{L^2(\mathbb{R}^n)}=0.\]
\end{prop}

\begin{proof}
This proof works analogously to the proof of  Equation (5.5) in \cite{hofmann_lp_2022}. Note that the uniform support of \(f_s\) ensures that the support of the chosen \(\varphi_\epsilon^s\) is also subset of \(K\) and has uniformly bounded measure.
\end{proof}








We have the two following important results
\begin{prop}\label{Proposition11}[Proposition 11 in \cite{hofmann_dirichlet_2022}]
    Let \(\eta>0,\alpha>0\) and L be t-independent. Then we have for all \((y,t)\in\Gamma_{\eta\alpha}(x)\)
    \[\eta^{-1}\partial_t e^{-(\eta t)^2L}f(y)\lesssim M(\nabla f)(x),\]
    and hence
    \[\Vert \eta^{-1} N_{\eta\alpha}[\partial_t e^{-(\eta t)^2L}f]\Vert_{L^p}\lesssim \Vert\nabla f\Vert_{L^p}\]
    for all \(p>1\) and \(f\in W^{1,p}(\mathbb{R}^n)\).
\end{prop}

For us relevant is the adaptation to our case without t-independent L.

\begin{cor}\label{cor:PointwiseBoundsofw_tAndrhoByM(nablaphi^s)}
    Let \(\eta>0,\alpha>0\). Then we have for all \((y,t)\in\Gamma_{\eta\alpha}(x)\)
    \begin{align} \eta^{-1}w_t(y,s)=sL^se^{-(\eta s)^2L^s}\phi^s\lesssim M(\nabla \phi^s)(x),\label{eq:w_tpointwiseBounded}\end{align}
    and
    \begin{align}\frac{\rho_\eta(y,s)}{\eta s}=\frac{e^{-(\eta s)^2L^s}(\phi^s-m)(y)}{s}\lesssim M(\nabla \phi^s)(x),\label{eq:rhopointwiseBounded}\end{align}
    where
    \[m(s):=\fint_{B_x(x, 2\eta\alpha s)}\phi^s(x) dx=(\phi^s(\cdot))_{B_x(x, 2\eta\alpha s)}.\]
\end{cor}

\begin{proof}
    The first inequality \eqref{eq:w_tpointwiseBounded} follows directly from \refprop{Proposition11}. For \eqref{eq:rhopointwiseBounded} we can observe in the proof of \refprop{Proposition11} that the only properties of \(\partial_t e^{-t^2L}\) that were used are bounds of its kernel which can be found in Proposition 4.3 of \cite{hofmann_lp_2022}. However, the same Proposition gives the same bounds for \(\frac{e^{-t^2L}}{t}\) and hence we get with a similar proof to that of \eqref{eq:w_tpointwiseBounded} also \eqref{eq:rhopointwiseBounded}. 
\end{proof}

\begin{prop}[Proposition 12 in \cite{hofmann_dirichlet_2022}]\label{Proposition12}
     Let \(\eta>0\) and \(L\) be t-independent. Then we have 
    \[\Vert \tilde{N}_\eta[\nabla e^{-(\eta t)^2L}f]\Vert_{L^p}\lesssim \Vert\nabla f\Vert_{L^p}\]
    for all \(p>2\) and \(f\in W^{1,p}(\mathbb{R}^n)\).
\end{prop}

We will also apply the following very basic lemma which can be proved with the above introduced statements and ideas.

\begin{lemma}\label{lemma:nablaSemigroupBoundedByNablaf}
Furthermore for t-independent \(L\), if \(f\in W_0^{1,2}(\mathbb{R}^n)\) then 
\[\Vert \nabla e^{-tL}f\Vert_{L^2(\mathbb{R}^n)}\leq C \Vert \nabla f\Vert_{L^2(\mathbb{R}^n)},\]
and
\[\Vert \nabla \partial_t e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}\leq C t^{-1}\Vert \nabla f\Vert_{L^2(\mathbb{R}^n)}\]
\end{lemma}

\begin{proof}
    The first inequality is an easy corollary from the Kato conjecture, i.e. we have with \refprop{prop:KatoConjecture} and \refprop{prop:L2NormBoundsOfHeatSemigroup}
    \begin{align*}
        \Vert \nabla e^{-tL}f\Vert_{L^2(\mathbb{R}^n)}&\lesssim \Vert L^{1/2} e^{-tL}f\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert  e^{-tL}L^{1/2} f\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\lesssim \Vert L^{1/2} f\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert  \nabla f\Vert_{L^2(\mathbb{R}^n)}.
    \end{align*}
    For the second one we have
    \begin{align*}
        \Vert\nabla \partial_t e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}^2 &\lesssim \int_{\mathbb{R}^n} A\nabla \partial_t e^{-t^2L}f \cdot \nabla \partial_t e^{-t^2L}f dx
        \\
        &\lesssim \int_{\mathbb{R}^n} \frac{\partial_{tt} e^{-t^2L}f}{2t}\partial_t e^{-t^2L}f dx
        \\
        &\lesssim \frac{1}{t}\Vert\partial_{tt} e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)} \Vert\partial_t e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}
    \end{align*}
    Again, we can observe in the proof of in \refprop{Proposition11} that the only properties of \(\partial_t e^{-t^2L}\) that were used are bounds of its kernel which can be found in Proposition 4.3 of \cite{hofmann_lp_2022}. However, the same Proposition gives the same bounds for \(t\partial_{tt}e^{-t^2L}\) and hence we get 
    \[\Vert\partial_{tt} e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}\lesssim \frac{1}{t}\Vert\nabla f\Vert_{L^2(\mathbb{R}^n)}\qquad\textrm{and}\qquad \Vert\partial_{t} e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert\nabla f\Vert_{L^2(\mathbb{R}^n)}.\]
    So in total we have
    \[ \Vert\nabla \partial_t e^{-t^2L}f\Vert_{L^2(\mathbb{R}^n)}^2\lesssim \frac{1}{t^2}\Vert\nabla f\Vert_{L^2(\mathbb{R}^n)}^2.\]
\end{proof}



\begin{comment}
Next, we would like to recall \(L^2\) off-diagonal estimates for the heat semigroup. We say that an operator family \(\mathcal{T}_t:L^2\to L^2\) satisfies an \(L^2- L^2\) off-diagonal estimate, if for all closed sets \(E,F\subset \mathbb{R}^n\) and \(h\in L^2(\mathbb{R}^n)\) with support in \(E\)
\[\Vert T_t(h)\Vert_{L^2(F)}\leq C e^{-\frac{c\Dist(E,F)^2}{t}}\Vert h\Vert_{L^2(E)}\]
holds. Note that this definition can be made more general for \(L^p-L^q\) off-diagonal estimates (cf. \cite{hofmann_lp_2022}). However, we just need the \(L^2\) version. 

\begin{prop}[Proposisiton 4.38 in \cite{hofmann_lp_2022}]
    Let L be t-independent.
    The operator family \((\sqrt{t}e^{-tL})_{t>0}\) satisfies \(L^2-L^2\) off-diagonal estimates, i.e.
    \[\Vert e^{-tL}(h)\Vert_{L^2(F)}\leq C \frac{1}{\sqrt{t}}e^{-\frac{c\Dist(E,F)^2}{t}}\Vert h\Vert_{L^2(E)}\]
    for all \(h\in L^2(E)\).
\end{prop}

There are also off-diagonal estimates for \(e^{-tL}\) and \(\partial_te^{-tL}\), and the reader could look them up in \cite{hofmann_lp_2022}.

\end{comment}

==> KatoPrelims.tex <==
\section{Consequences of the Kato conjecture}


The following result can be found as Theorem 4.77 in \cite{hofmann_lp_2022}. Note that we define \(\dot W^{1,p}(\mathbb{R}^n)\) as the closure of \(C_0^\infty(\mathbb{R}^n)\) under the seminorm given by \(\Vert f\Vert_{\dot W^{1,p}}:=\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\).
\begin{prop}\label{prop:KatoConjecture}
    For a function \(f\in \dot W^{1,p}(\mathbb{R}^n)\) we have
    \[\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\]
    for all \(1<p<\infty\). Furthermore, there exists \(\varepsilon_1>0\) such that if \(1<p<2+\varepsilon_1\) then
    \[\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}.\]
\end{prop}

A direct consequence is the following corollary 
\begin{cor}\label{cor:NablaL^-1/2Bounded}
    For a function \(f\in L^2(\mathbb{R}^n)\) we have
    \[\Vert \nabla L^{-1/2} f\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}\]
    and if f is a vector valued function
    \[\Vert L^{-1/2} \Div(f)\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}.\]
\end{cor}

==> NontangentialBounds.tex <==
\section{Bounds on the Nontangential Maximal Function}



==> NotationsAndSetting.tex <==
\section{Notations and Setting}

\begin{comment}
Let \(\Omega:=\mathbb{R}^{n+1}_+:=\mathbb{R}^n\times [0,\infty)\) be the upper half space and \(\mathcal{L}:=\Div(A\nabla\cdot)\) an uniformly elliptic operator, i.e. there exists \(\lambda_0>0\)
\begin{align}
    \lambda_0 |\xi|^2\leq \xi^T A(x) \xi \leq \lambda_0^{-1}|\xi|^2 \qquad \textrm{ for all }\xi\in \mathbb{R}^{n+1}\textrm{, and a.e. }x\in \mathbb{R}^{n+1}_+.
\end{align}

\smallskip
\end{comment}

Throughout this work \(\Delta=\Delta(P,r):=B(P,r)\cap\partial\Omega\) denotes a boundary ball centered in point \(P\in\partial\Omega\) with radius \(l(\Delta)=r>0\) and 
\[T(\Delta):=\{(x,t)\in\Omega; x\in\Delta, 0<t<l(\Delta)\}\]
its Carleson region. 
The cone with vertex in \(P\in \partial\Omega\) and aperture \(\alpha\) is denoted by
\[\Gamma_\alpha(P):=\{(x,t)\in \Omega; |x-P|<\alpha t\}.\] 
For an open set \(F\subset \Delta\) we define the saw-tooth region \(\Omega_\alpha(F):=\bigcup_{P\in F}\Gamma_\alpha(P)\) and the truncated saw-tooth region \(\tilde{\Omega}_\alpha(F):=\Omega_\alpha(F)\cap T(\Delta)\).
Furthermore, we set \(\mathcal{D}^\eta_k(\Delta)\) as the collection of certain boundary balls with radius radius \(\eta 2^{-k}\) in \(\Delta\) such that their union covers \(\Delta\) but they have finite overlap. %The boundary balls in \(\mathcal{D}^\eta_k(\Delta)\) are a decomposition of \(\Delta\).

\smallskip

We define the nontangential maximal function as
\[N_\alpha(u)(P):=\sup_{(x,t)\in \Gamma_\alpha(P)} |u(x,t)|\qquad \textrm{ for }P\in \mathbb{R}^n,\]
and the mean-valued nontangential maximal function as
\[\tilde{N}_\alpha(u)(P):=\sup_{(x,t)\in \Gamma_\alpha(P)} \Big(\int_{\big\{(y,s); |y-x|<\frac{t}{2}\big\}}|u(y,s)|^2dyds\Big)^{1/2}\qquad \textrm{ for }P\in \mathbb{R}^n.\]

\smallskip

We can now consider the \(L^p\)-Dirichlet boundary value problem.
\begin{defin}\label{def:L^pDirichletProblem}
We say the \textit{\(L^p\)-Dirichlet boundary value problem} is solvable for \(\mathcal{L}\) if for all boundary data \(f\in C_c(\partial\Omega)\cap L^p(\Omega)\) the unique existent solution \(u\in W^{1,2}(\Omega)\) of 
\[\begin{cases} \mathcal{L}u=0 &\textrm{in }\Omega, \\ u=f &\textrm{on }\partial\Omega.\end{cases}\]
satisfies
\[\Vert N(u) \Vert_{L^p(\partial\Omega)}\leq C \Vert f\Vert_{L^p(\partial\Omega)},\]
where the constant \(C\) is independent of \(u\) and \(f\).
\end{defin}
As usual, we denote the elliptic measure by \(\omega\), the usual \(n\)-dimensional Hausdorff surface measure by \(\sigma\) and the Muckenhoupt and Reverse Hölder spaces by \( A_\infty(d\sigma)\) and \(B_q(d\sigma)\) respectively. The solvability of the \(L^p\) Dirichlet boundary value problem is equivalent to \(\omega\in B_{p'}(d\sigma)\), which means that solvability for some \(p\) is equivalent to \(\omega\in A_\infty(d\sigma)\). 

\medskip

In our setting we would like to introduce a bit more notation and specification. In the following we are 
considering the matrix
\begin{align} 
A(x,t)=\begin{pmatrix} \AP(x,t) & b(x,t) \\ c(x,t) & d(x,t)\end{pmatrix}\label{eq:DefinitionOfMatrixA}
\end{align}
for \((x,t)\in \Omega=\mathbb{R}^{n+1}_+\), where \(\AP\) is the upper n times n block of \(A\) and \(b,c,d\) are vector functions to \(\mathbb{R}^n\) or \(\mathbb{R}\) respectively. We are discussing the operator \(Lu(x,t):=\Div_x(A(x,t)\nabla_x u(x,t))\) for \(u\in W^{1,2}(\Omega)\) and the family of operators
\[L^sv(x):=\Div_x(\AP(x,s)\nabla_x v(x)) \qquad\textrm{ for }v\in W^{1,2}(\partial\Omega)=W^{1,2}(\mathbb{R}^n), s>0.\]
We tend to write \(\nabla=\nabla_x\) suppressing the index when dealing with the gradient only in the components of \(x\) and will clarify with \(\nabla_{x,t}\) where we mean the full gradient.

At last, we notice that from \(\frac{|\partial_t A|}{t}\leq C\) and the mixed \(L^1-L^\infty\) Carleson type condition (\ref{condition:L^1Carlesontypecond}), which is
\begin{align*}\int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty ds\leq C<\infty,\end{align*}
we can deduce a mixed \(L^2-L^\infty\) Carleson type condition
\begin{align}
    \int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty^2 s ds\leq C<\infty.\label{condition:L^2Carlesontypecond}
\end{align}

A technical result we will need is the following lemma.
\begin{lemma}[\cite{Giaquinta+1984} Chapter V Lemma 3.1]\label{lemma:LEMMA5}
    Let \(f(t)\) be a nonnegative bounded function in \([r_0,r_1], r_0\geq 0\). Suppose that for \(r_0\leq s<t\leq r_1\) we have
    \[f(s)\leq (A(s-t)^{-\alpha}+B)+\sigma f(t)\]
    where \(A,B,\sigma, \alpha\) are nonnegative constants with \(0\leq \sigma<1\). Then for all \(r_0\leq \rho<R\leq r_1\) we have
    \[f(\rho)\leq c(A(R-\rho)^{-\alpha}+B)\]
    where c is a cosntant depending on \(\alpha\) and \(\sigma\).
\end{lemma}




==> SquareFunctionBoundsOfThePartialDerivativesOftheta.tex <==
\section{Square function bounds on the parts of the derivative of \(\theta\)}

We investigate square function type expression involving of \(\partial_s\phi^s,w_t,w_s^{(1)}\) and \(w_s^{(2)}\). 

\subsection{The partial derivative parts \(\partial_s\phi^s\) and \(w_s^{(1)}\)}

Instead of investigating \(\partial_s\phi^s\) and \(w_s^{(1)}\) separately, we are also going to use that their difference
\[\partial_s\phi^s-w_s^{(1)}=\partial_s\phi^s-e^{-(\eta s)^2L^s}\partial_s\phi^s\]
gives us better properties.

\begin{lemma}\label{lemma:SqFctBoundsForpartial_sPhiAndw_s^1}
If we assume \eqref{condition:L^2Carlesontypecond}, the following square function bounds hold
\begin{enumerate}[(1)]
    \item \[\Big\Vert\Big(\int_0^\infty\frac{|\partial_s\phi^s-w_s^{(1)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|,\]\label{lemma:w_s^1SqFctBound1}
    \item \[\Big\Vert\Big(\int_0^\infty\frac{|s\nabla\partial_s\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}+\Big\Vert\Big(\int_0^\infty\frac{|s\nabla w_s^{(1)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|.\label{lemma:w_s^1SqFctBound2}\]
\end{enumerate}
\end{lemma}

\begin{proof}
    For \eqref{lemma:w_s^1SqFctBound1} we use an analogous way to the proof of \reflemma{lemma:thetaPointwiseBoundOnGoodSetF}, where we use \refprop{Proposition11} to get
    \begin{align*}
        (\partial_s\phi^s-e^{-(\eta s)^2L^s}\partial_s\phi^s)(x)&=\int_0^s\partial_t e^{-(\eta t)^2L^s}\partial_s \phi^sdt\lesssim \eta\int_0^s M[\nabla\partial_s\phi^s](x)dt
        \\
        &\lesssim M[\nabla\partial_s\phi^s](x)\eta s.
    \end{align*}
    Hence,
    \begin{align*}
        \Big\Vert\Big(\int_0^\infty\frac{|\partial_s\phi^s-w_s^{(1)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}&\lesssim \int_0^\infty \int_{\mathbb{R}^n}|M[\nabla\partial_s\phi^s](x)|^2sdxds
        \\
        &\lesssim \int_0^\infty \Vert\nabla\partial_s\phi^s\Vert_{L^2(\mathbb{R}^n)}^2sds,
    \end{align*}
    
    and with \eqref{equation:L2ofpartial_snablaphiBounded} we get \(\int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty^2 |\Delta| s ds\).

    \hfill\\
    For \eqref{lemma:w_s^1SqFctBound2} we just observe that \(\Vert\nabla w_s^{(1)}\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert \nabla\partial_s\Phi^s\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert\partial_s A(\cdot,s)\Vert_\infty^2 |\Delta|\), which implies
    \begin{align*}
        \Big\Vert\Big(\int_0^\infty\frac{|s\nabla\partial_s\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}&,\Big\Vert\Big(\int_0^\infty\frac{|s\nabla w_s^{(1)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\qquad\qquad\lesssim \int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty^2 |\Delta| s ds.
    \end{align*}
    
\end{proof}









































\subsection{The partial derivative part \(w_s^{(2)}\)}

\begin{lemma}\label{lemma:w_s^2/nablaw_s^2spatialL^2Bound}
    It holds that
    \begin{enumerate}
        \item \[\Vert w_s^{(2)}(\cdot,s)\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert \partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}s,\]\label{lemma:w_s^2spatialL^2Bound}
        \item \[\Big\Vert\Big(\int_0^\infty\frac{|w_s^{(2)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}^2\lesssim |\Delta|.\]\label{lemma:w_s^2SqFctBound1}
    \end{enumerate}
\end{lemma}

\begin{proof}
    We begin by proving \eqref{lemma:w_s^2spatialL^2Bound}. By Minkowski inequality, we obtain
    \begin{align*}
        &\Big\Vert\int_0^{s} \eta^2\tau e^{-\eta^2(s^2-\tau^2)L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))d\tau\Big\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\qquad =\int_0^{s} \Vert\eta^2\tau e^{-\eta^2(s^2-\tau^2)L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)} d\tau.
    \end{align*}
    We introduce a reparametrisation \(r:=\sqrt{s^2-\tau^2}\) or equivalently \(\tau=\sqrt{s^2-r^2}\). Applying this change of variables leads to
    \begin{align*}
        &\int_0^{s} \Vert\eta^2\tau e^{-\eta^2(s^2-\tau^2)L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)} d\tau
        \\
        &\qquad=\int_0^{s} \Vert\eta^2 r e^{-\eta^2r^2L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)} dr
        \\
        &\qquad =\int_0^{s} \Vert\eta^2 \partial_r e^{-\eta^2r^2L^s}(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)} dr.
    \end{align*}

    According to \refprop{Proposition11} we have 
    \begin{align*}
        &\Vert\eta^2 \partial_r e^{-\eta^2r^2L^s}(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\qquad \lesssim\big\Vert\eta^2 M\big[\nabla(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\big]\big\Vert_{L^2(\mathbb{R}^n)}.
    \end{align*}
    Next, we can use the boundedness of the Hardy-Littlewood Maximal function and the boundedness of the operator \(\nabla (L^s)^{-1}\Div\)  and \reflemma{lemma:nablaSemigroupBoundedByNablaf} which yield
        \begin{align*}
            &\big\Vert\eta^2 M\big[\nabla(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\big]\big\Vert_{L^2(\mathbb{R}^n)}
            \\
            &\qquad\lesssim \Vert\eta^2\nabla(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)}
            \\
            &\qquad\lesssim \Vert\eta^2\partial_s A(\cdot,s)\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)}
            \\
            &\qquad\lesssim \eta^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}\Vert\nabla w(x,\eta^2(s^2-r^2),s))\Vert_{L^2(\mathbb{R}^n)}
            \\
            &\qquad\lesssim \eta^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}\Vert\nabla \phi^s\Vert_{L^2(\mathbb{R}^n)}
            \\
            &\qquad\lesssim \eta^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}.
    \end{align*}
    Hence we get in total
    \[\Vert w_s^{(2)}(\cdot,s)\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert \partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}s.\]

    At last, we get \eqref{lemma:w_s^2SqFctBound1} as an easy consequence of \eqref{lemma:w_s^2spatialL^2Bound} and \eqref{condition:L^2Carlesontypecond}, since
    \[\Big\Vert\Big(\int_0^\infty\frac{|w_s^{(2)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim \int_0^\infty\Vert \partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2|\Delta|s ds\lesssim |\Delta|.\]


\end{proof}

\begin{lemma}\label{lemma:SqFctBoundsForw_s^2}
Let \(Q\subset \partial\Omega\) be a boundary cube of size s, i.e. \(l(Q)\approx s\), \((t_j)_{j\in\Z}=(2^{j})_{j\in\Z}\) be a dyadic partition of \((0,\infty)\), and the index \(i\) such that \(s\in (t_i,t_{i+1})\). If we assume \eqref{condition:L^2Carlesontypecond}, we have the following local bound involving \(w_s^{(2)}\)
\begin{align}
    \int_Q |\nabla w_s^{(2)}(x,s)|^2dx&\lesssim \frac{1}{s^2}\fint_{t_{i-1}}^{t_{i+2}}\int_{2Q}|v(x,k,s)|^2dkdx\nonumber
    \\
    &\qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\fint_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-t^2L^s}\phi_s|^2dxdt \nonumber
    \\
    &\qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \fint_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk.\label{lemma:localEstimateNablaw_s^2}
\end{align}
As a consequence we have 
\begin{align}
    \Vert \nabla w_s^{(2)}\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert \partial_s A(\cdot, s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}\label{lemma:Nablaw_s^2SpatialBound},
\end{align}
and the square function bound
\begin{align}
    \Big\Vert\Big(\int_0^\infty\frac{|s\nabla w_s^{(2)}|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|.\label{lemma:w_s^2SqFctBound2}
\end{align}

\end{lemma}

\begin{proof}
In this proof we are going to use the notation of \reflemma{Lemma:CacciopolliTypeInequalities}. Let \((t_j)_{j\in\Z}\) be a dyadic partition of \((0,\infty)\) and the index \(i\) such that \(s\in (t_i,t_{i+1})\).
We begin with the use of the fundamental theorem for calculus and Jenssen's inequality to obtain
\begin{align*}
    \int_Q |\nabla w_s^{(2)}(x,s)|^2 dx &= \int_Q |\nabla v(x,s,s)|^2 dx  = \fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,s,s)|^2dtdx
    \\
    &=\fint_{t_i}^{t_i+1}\int_Q \Big|\nabla v(x,t,s) + \int_t^s\nabla\partial_k v(x,k,s)dk\Big|^2dtdx
    \\
    &\lesssim\fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,t,s)|^2 dxdt
    \\
    &\qquad + \fint_{t_i}^{t_i+1}|s-t|\int_Q\int_t^s|\nabla \partial_k v(x,k,s)|^2dkdtdx
    \\
    &\lesssim\fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,t,s)|^2 dxdt
    \\
    &\qquad  + s\int_Q\int_{t_i}^{t_{i+1}}|\nabla\partial_k v(x,k,s)|^2dkdx=I_1+sI_2
\end{align*}
For \(I_1\) we get by Caccioppolli type inequality \reflemma{Lemma:CacciopolliTypeInequalities}
\[I_1\lesssim \frac{1}{s^2}\fint_{t_{i-1}}^{t_{i+2}}\int_{2Q}|v(x,t,s)|^2dxdt + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty}^2\fint_{t_{i-1}}^{t_{i+2}}\int_{2Q}|\nabla e^{-t^2L^s}\phi_s|^2dxdt.\]

For \(I_2\) we apply \reflemma{Lemma:CacciopolliTypeInequalities} first to get
\begin{align*}
    I_2&\lesssim\frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-1}}^{t_{i+2}}\int_{2Q}|\nabla e^{-t^2L^s}\phi_s|^2dxdt
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-1}}^{t_{i+2}}\int_{\frac{5}{4}Q} |\nabla \partial_t e^{-t^2L^s}\phi_s|^2dxdt
    \\
    &\qquad+ \frac{1}{s^2}\int_{t_{i-1}}^{t_{i+2}}\int_{\frac{5}{4}Q} |\partial_k v(x,k,s)|^2 dxdk
\end{align*}
Further, we will have to apply \reflemma{lemma:LEMMA5}. Hence we have to introduce the smooth cut-off function \(\eta\) and choose \(\frac{5}{4}\leq\EPS_1<\EPS_2\leq\frac{3}{2}\), \(d:=(\EPS_2-\EPS_1)/2\), i.e. \(\eta\equiv 1\) on \(\EPS_1 Q\times[\frac{1}{\EPS_1}t_{i-1},\EPS_1t_{i+2}]\) and \(\eta\equiv 0\) on \(\Omega\setminus (\EPS_2 Q\times [\frac{1}{\EPS_2}t_{i-2},\EPS_2 t_{i+3}])\) with \(|\nabla \eta|\lesssim \frac{1}{ds}\), where we set
\begin{align*}
&Q^*:=\EPS_1 Q\times[\frac{1}{\EPS_1}t_{i-1},\EPS_1t_{i+2}],\qquad \tilde{Q}^*:=(\EPS_1+d) Q\times[\frac{1}{\EPS_1+d}t_{i-1},(\EPS_1+d)t_{i+2}], 
\\
&\hat{Q}^*:=\EPS_2 Q\times[\frac{1}{\EPS_2}t_{i-1},\EPS_2t_{i+2}].
\end{align*}

Then we have

\begin{align*}
    &\int_{Q^*}|\partial_k v(x,k,s)|^2dkdx=\int_{\tilde{Q}^*}\int_{\EPS_2 Q}\partial_k v\big(2kL^s v + k\Div(\partial_s A\nabla e^{-k^2L^s}\phi_s)\big)\eta^2 dkdx 
    \\
    &\qquad=\int_{\tilde{Q}^*}\nabla \partial_k v \nabla v\eta^2kdxdk + \int_{\tilde{Q}^*}\nabla \partial_k v \partial_s A\nabla e^{-k^2L^s}\phi_s\eta^2kdxdk
    \\
    &\qquad\quad + \int_{\tilde{Q}^*} \partial_k v \nabla v\nabla\eta^2kdxdk + \int_{\tilde{Q}^*} \partial_k v \partial_s A\nabla e^{-k^2L^s}\phi_s\nabla\eta^2kdxdk
    \\
    &\qquad=: II_1+II_2+II_3+II_4.
\end{align*}
We estimate each integral separately using the same techniques consisting of Hölder's inequality, \reflemma{Lemma:CacciopolliTypeInequalities}, \reflemma{lemma:UnifromBoundOnrholocally} and hiding of terms on the left hand side. At this point, we will be more precise and show these calculations for all terms. First, for \(II_1\)
\begin{align*}
    II_1&\lesssim s\Big(\int_{\tilde{Q}^*}|\nabla v|^2dxdk\Big)^{1/2}\Big(\int_{\tilde{Q}^*}|\nabla\partial_k v|^2dxdk\Big)^{1/2}
    \\
    &\lesssim s\Big(\frac{1}{d^2s^2}\int_{\hat{Q}^*}|v(x,k,s)|^2dxdk + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk\Big)^{1/2}
    \\
    &\quad\cdot \Big(\frac{1}{d^2s^2}\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^2s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk\Big)^{1/2}
    \\
    &\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^4s^2}\int_{\tilde{Q}^*}|v(x,k,s)|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
\end{align*}

Furthermore, we have
\begin{align*}
    II_2&\lesssim \sigma d^2s^2\int_{\tilde{Q}^*}|\nabla \partial_k v|^2dxdk + \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\tilde{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \big(\frac{1}{d^2}+1\big)\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}
and
\begin{align*}
    II_3&\lesssim \sigma \int_{\tilde{Q}^*}|\partial_k v|^2dxdk + \frac{C_\sigma}{d^2}\int_{\tilde{Q}^*}|\nabla v|^2dxdk
    \\
    &\lesssim \sigma \int_{\hat{Q}^*}|\partial_k v|^2dxdk + \frac{1}{d^4s^2}\int_{\hat{Q}^*}\int_{2Q}|v(x,k,s)|^2dxdk
    \\
    &\qquad+ \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}
and
\begin{align*}
    II_4\lesssim \sigma \int_{\tilde{Q}^*}|\partial_k v|^2dxdk + \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\tilde{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk.
\end{align*}

Putting all these integrals together we obtain 
\begin{align*}
    \int_{\tilde{Q}^*}|\partial_k v|^2dxdk&\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^4s^2}\int_{\tilde{Q}^*}|v(x,k,s)|^2dxdk
    \\
    &\qquad + \big(1+\frac{1}{d^2}\big)\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
\end{align*}

which leads with \reflemma{lemma:LEMMA5} to
\begin{align*}
    I_2&\lesssim\frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{\frac{5}{4}Q} |\nabla \partial_k e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad+ \frac{1}{s^2}\int_{t_{i-2}}^{t_{i+3}}\int_{\frac{5}{4}Q} |\partial_k v(x,k,s)|^2 dxdk
    \\
    &\lesssim \frac{1}{s^4}\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad + \frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}

and hence
\begin{align*}
    \int_Q |\nabla w_s^{(2)}(x,s)|^2dx&=I_1+sI_2
    \\
    &\lesssim \frac{1}{s^3}\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad + \frac{1}{s}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad+  s\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk.
\end{align*}




Now, we can show the global estimates (\ref{lemma:Nablaw_s^2SpatialBound}) and (\ref{lemma:w_s^2SqFctBound2}). We use above introduced partition of \((t_j)_j\) and set \(\mathcal{D}_j\) as the collection of a decomposition of \(3\Delta\) into cubes \(Q\) of size \(l(Q)\approx t_j\). First for (\ref{lemma:Nablaw_s^2SpatialBound}) we have for \(s\approx t_i\)
\begin{align*}
    &\int_{\mathbb{R}^n} |\nabla w_s^{(2)}(x,s)|^2 sdxds\leq \sum_{Q\in \mathcal{D}_j} |\nabla w_s^{(2)}(x,s)|^2 sdxds
    \\
    &\qquad\lesssim \sum_{Q\in \mathcal{D}_j}\Big(\frac{1}{s^2}\fint_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad\qquad+  s^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk\Big)
    \\
    &\qquad\lesssim \frac{1}{s^2}\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|v(x,k,s)|^2dkdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad\qquad+  s^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk\Big).
\end{align*}

We note here that due to \reflemma{lemma:nablaSemigroupBoundedByNablaf} and (\ref{equation:L2ofnablaphiBounded})
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-2}}^{t_{i+3}}\int_{\mathbb{R}^n}|\nabla e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|,\]
and
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|.\]

Since we can also proof 
\[\int_{\mathbb{R}^n}|v(x,t,s)|^2dx\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s^2 \]
analogously to the proof of \ref{lemma:w_s^2spatialL^2Bound} in \reflemma{lemma:w_s^2/nablaw_s^2spatialL^2Bound}, we obtain 

\begin{align*}
    \int_{3\Delta} |\nabla w_s^{(2)}(x,s)|^2 sdxds\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2|\Delta|,
\end{align*}
which yields (\ref{lemma:Nablaw_s^2SpatialBound}). At last, (\ref{lemma:w_s^2SqFctBound2}) is direct consequence of (\ref{lemma:Nablaw_s^2SpatialBound}). To see this we note with (\ref{condition:L^2Carlesontypecond}) 
\begin{align*}
    \int_0^\infty \int_{\mathbb{R}^n} |\nabla w_s^{(2)}(x,s)|^2 sdxds \lesssim |\Delta|\int_0^\infty \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2s ds.
\end{align*}




\begin{comment}
Then
\begin{align*}
    \int_{3\Delta}\int_0^\infty |\nabla w_s^{(2)}(x,s)|^2 sdxds\leq \sum_{j, Q\in \mathcal{D}_j}\int_Q\int_{t_i}^{t_{i+1}} |\nabla w_s^{(2)}(x,s)|^2 sdxds.
\end{align*}
We can apply the local estimate (\ref{lemma:localEstimateNablaw_s^2}) to obtain
\begin{align*}
    &\sum_{j, Q\in \mathcal{D}_j}\int_Q\int_{t_i}^{t_{i+1}} |\nabla w_s^{(2)}(x,s)|^2 sdxds
    \\
    &\lesssim \sum_{j, Q\in \mathcal{D}_j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{Q}|v(x,t,s)|^2dtdx
    \\
    &\qquad \qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{Q}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds
    \\
    &\lesssim \sum_{j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|v(x,t,s)|^2dtdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta} |\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds.
\end{align*}
We note here that due to \reflemma{lemma:nablaSemigroupBoundedByNablaf} and (\ref{equation:L2ofnablaphiBounded})
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|\nabla e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|,\]
and
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \fint_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|.\]

Since we can also proof 
\[\int_{3\Delta}|v(x,t,s)|^2dx\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s^2 \]
analogously to the proof of \ref{lemma:w_s^2spatialL^2Bound} in \reflemma{lemma:w_s^2/nablaw_s^2spatialL^2Bound}, we get in total

\begin{align*}
    &\sum_{j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|v(x,t,s)|^2dtdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds.
    \\
    &\lesssim \sum_j\int_{t_i}^{t_{i+1}} \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s ds= \int_0^\infty \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s ds.
\end{align*}
\end{comment}









\end{proof}




\begin{comment}
 \begin{lemma}\label{Lemma:CacciopolliTypeInequalities}
     Let \(2\hat{Q}\subset \Omega\) be a Whitney cube, i.e. \(\mathrm{dist}(\hat{Q},\partial\Omega)\approx l(\hat{Q})\approx s\).
     If we set 
     \[v(x,t,s):=v_2(x,t^2,s)=\int_0^t 2\tau e^{-(t^2-\tau^2)L^s}\Div(\partial_s A(x,s)\nabla e^{-\tau^2 L^s}\phi_s(x))d\tau,\]
     then we have
     \[\int_{\hat{Q}} |\nabla_x v(x,t,s)|^2dxdt\lesssim \frac{1}{s^2}\int_{2\hat{Q}}|v(x,t,s)|^2dxdt + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt,\]
     and
     \begin{align*}
         \int_{\hat{Q}} |\nabla_x\partial_t v(x,t,s)|^2dxdt&\lesssim \frac{1}{s^2}\int_{2\hat{Q}}|\partial_t v(x,t,s)|^2dxdt
         \\
         & \qquad + \frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt
         \\
         &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2Q}|\nabla\partial_te^{-t^2L^s}\phi_s|^2dxdt.
     \end{align*}
 \end{lemma}
\end{comment}

\begin{comment}
\begin{proof}
    First we denote \(\tilde{v}:=\partial_t v\) to shorten notation. We observe that \(v\) and \(\tilde{v}\) satisfy the following PDEs
    \begin{align*}
        \partial_t v &= 2t\Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) - \int_0^t 4t\tau L^se^{-(t^2-\tau^2)L^s}\Div(\partial_s A(x,s)\nabla e^{-\tau^2 L^s}\phi_s(x))d\tau
        \\
        &= 2t\Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) - 2t L^s v,
    \end{align*}
    and
    \begin{align*}
        \partial_t \tilde{v} &= \Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) + 2t\Div(\partial_s A\nabla\partial_t e^{-t^2L^s}\phi_s) - 2 L^s v - 2t L^s \tilde{v}.
    \end{align*}

    The rest of the proof is a standard Cacciopolli inequality proof for inhomogeneous parabolic PDEs.


    Let \(\eta\) be a smooth cut-off with \(\eta\equiv 1\) on \(\hat{Q}\) and \(\eta\equiv 0\) on \(\Omega\setminus 2\hat{Q}\) with \(|\nabla \eta+\partial_t\eta|\lesssim \frac{1}{s}\). First for \(v\), we calculate

    \begin{align*}
        \int_{\hat{Q}} |\nabla v(x,t,s)|^2dxdt&\leq \int_{2\hat{Q}} A(x,s)\nabla v(x,t,s)\cdot \nabla v(x,t,s) \eta^2(x,t)dxdt
        \\
        &=\int_{2\hat{Q}} L^s\nabla v(x,t,s) \nabla v(x,t,s) \eta^2(x,t)dxdt 
        \\
        &\qquad- \int_{2\hat{Q}} A(x,s)\nabla v(x,t,s)\cdot v(x,t,s) \nabla\eta^2(x,t)dxdt=:I_1+I_2
    \end{align*}
    For \(I_2\) we directly get for a small \(\sigma\)
    \[I_2\lesssim \Big(\int_{2\hat{Q}}|\nabla v\eta|^2\Big)^{1/2}\Big(\int_{2\hat{Q}}|\nabla\eta v|^2\Big)^{1/2}\lesssim \sigma\int_{2\hat{Q}}|\nabla v\eta|^2dxdt + C_\sigma\frac{1}{s^2}\int_{2\hat{Q}}|v|^2dxdt,\]
    and can hide the first term on the left side.

    For \(I_1\) we have
    \begin{align*}
       I_1&\lesssim -\frac{1}{s}\int_{2\hat{Q}}\partial_t v v \eta^2 dxdt + \int_{2\hat{Q}} 2\Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) v\eta^2dxdt
       \\
       &\lesssim \frac{1}{s}\int_{2\hat{Q}}\partial_t (v^2 \eta^2) dxdt + \frac{1}{s}\int_{2\hat{Q}} v^2 \partial_t\eta^2 dxdt
       \\
       & \qquad+ \int_{2\hat{Q}} 2\partial_s A\nabla e^{-t^2L^s}\phi_s (\nabla v\eta^2 + v\nabla\eta^2)dxdt
       \\
       &\lesssim \frac{1}{s^2}\int_{2\hat{Q}} |v|^2 dxdt + C_\sigma\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt + \sigma\int_{2\hat{Q}} |\nabla v|^2\eta^2 dxdt
    \end{align*}
    Hiding the last term on the left side gives in total
    \[\int_{\hat{Q}} |\nabla v(x,t,s)|^2dxdt\lesssim \frac{1}{s^2}\int_{2\hat{Q}} |v|^2 dxdt + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt,\]
    which completes the proof of the first Caccioppolli type inequality.

    \bigskip

    For the second one for \(\tilde{v}\) we proceed analogously with just more terms to handle. We have
    \begin{align*}
        \int_{\hat{Q}} |\nabla \tilde{v}(x,t,s)|^2dxdt&\leq \int_{2\hat{Q}} A(x,s)\nabla \tilde{v}(x,t,s)\cdot \nabla \tilde{v}(x,t,s) \eta^2(x,t)dxdt
        \\
        &=\int_{2\hat{Q}} L^s \tilde{v}(x,t,s) \tilde{v}(x,t,s) \eta^2(x,t)dxdt 
        \\
        &\qquad- \int_{2\hat{Q}} A(x,s)\nabla \tilde{v}(x,t,s)\cdot \tilde{v}(x,t,s) \nabla\eta^2(x,t)dxdt
        \\
        &=:II_1+II_2
    \end{align*}
    The term \(II_2\) works completely analogous to \(I_2\). For \(II_1\) however, we have
    \begin{align*}
       II_1&\lesssim \frac{1}{s}\int_{2\hat{Q}} 2\Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) \tilde{v}\eta^2dxdt + \int_{2\hat{Q}} 2\Div(\partial_s A\nabla \partial_t e^{-t^2L^s}\phi_s) \tilde{v}\eta^2dxdt
       \\
       &\qquad-\frac{1}{s}\int_{2\hat{Q}} L^s v \tilde{v}\eta^2 dxdt-\frac{1}{s}\int_{2\hat{Q}}\partial_t \tilde{v} \tilde{v} \eta^2 dxdt
       \\
       &\lesssim \frac{1}{s}\int_{2\hat{Q}} \partial_s A\nabla e^{-t^2L^s}\phi_s \nabla\tilde{v}\eta^2dxdt + \int_{2\hat{Q}} 2\partial_s A\nabla \partial_t e^{-t^2L^s}\phi_s \nabla\tilde{v}\eta^2dxdt
       \\
       &\qquad +\frac{1}{s}\int_{2\hat{Q}} \partial_s A\nabla e^{-t^2L^s}\phi_s \tilde{v}\nabla\eta^2dxdt + \int_{2\hat{Q}} 2\partial_s A\nabla \partial_t e^{-t^2L^s}\phi_s \tilde{v}\nabla\eta^2dxdt
       \\
       &\qquad-\frac{1}{s^2}\int_{2\hat{Q}}  \partial_t v \tilde{v}\eta^2 dxdt - \frac{1}{s}\int_{2\hat{Q}} 2\Div(\partial_s A\nabla e^{-t^2L^s}\phi_s) \tilde{v}\eta^2dxdt 
       \\
       &\qquad-\frac{1}{s}\int_{2\hat{Q}}\partial_t (\tilde{v}^2 \eta^2) dxdt +\frac{1}{s}\int_{2\hat{Q}}\tilde{v}^2 \partial_t \eta^2 dxdt.
    \end{align*}
    Here we did use the first PDE for \(v\) on the third term in the first inequality. Furthermore, we note that \(\partial_t v=\tilde{v}\) and proceeding with all the eight integrals in the from above known ways we get
    \begin{align*}
        II_1&\lesssim C_\sigma\frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt + \sigma \int_{2\hat{Q}} |\nabla \tilde{v}\eta|^2 dxdt
        \\
        &\qquad + C_\sigma\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla \partial_t e^{-t^2L^s}\phi_s|^2dxdt + \sigma\int_{2\hat{Q}} |\nabla \tilde{v}\eta|^2 dxdt
        \\
        &\qquad+ \frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla e^{-t^2L^s}\phi_s|^2dxdt + \frac{1}{s^2}\int_{2\hat{Q}} |\tilde{v}\eta|^2 dxdt
        \\
        &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{2\hat{Q}} |\nabla \partial_t e^{-t^2L^s}\phi_s|^2dxdt + \frac{1}{s^2}\int_{2\hat{Q}} | \tilde{v}\eta|^2 dxdt
        \\
        &\qquad + \frac{1}{s^2}\int_{2\hat{Q}} |\tilde{v}|^2 dxdt + \frac{1}{s^2}\int_{2\hat{Q}} |\tilde{v}|^2 dxdt.
    \end{align*}
    The last step requires hiding the terms with a small factor \(\sigma\) on the left side, which completes the proof.
    
\end{proof}
\end{comment}

\begin{comment}
\begin{proof}[Proof of \reflemma{lemma:SqFctBoundsForw_s^2}]
In this proof we are going to use the notation of \reflemma{Lemma:CacciopolliTypeInequalities}. Let \((t_j)_{j\in\Z}\) be a dyadic partition of \((0,\infty)\) and the index \(i\) such that \(s\in (t_i,t_{i+1})\).
We begin with the use of the fundamental theorem for calculus and Jenssen's inequality to obtain
\begin{align*}
    \int_Q |\nabla w_s^{(2)}(x,s)|^2 dx &= \int_Q |\nabla v(x,s,s)|^2 dx  = \fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,s,s)|^2dtdx
    \\
    &=\fint_{t_i}^{t_i+1}\int_Q \Big|\nabla v(x,t,s) + \int_t^s\nabla\partial_k v(x,k,s)dk\Big|^2dtdx
    \\
    &\lesssim\fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,t,s)|^2 dxdt
    \\
    &\qquad + \fint_{t_i}^{t_i+1}|s-t|\int_Q\int_t^s|\nabla \partial_k v(x,k,s)|^2dkdtdx
    \\
    &\lesssim\fint_{t_i}^{t_i+1}\int_Q |\nabla v(x,t,s)|^2 dxdt
    \\
    &\qquad  + s\int_Q\int_{t_i}^{t_{i+1}}|\nabla\partial_k v(x,k,s)|^2dkdx=I_1+sI_2
\end{align*}
For \(I_1\) we get by Caccioppolli type inequality \reflemma{Lemma:CacciopolliTypeInequalities}
\[I_1\lesssim \frac{1}{s^2}\fint_{t_{i-1}}^{t_{i+2}}\int_{2Q}|v(x,t,s)|^2dxdt + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty}^2\fint_{t_{i-1}}^{t_{i+2}}\int_{2Q}|\nabla e^{-t^2L^s}\phi_s|^2dxdt.\]

For \(I_2\) we apply \reflemma{Lemma:CacciopolliTypeInequalities} first to get
\begin{align*}
    I_2&\lesssim\frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-1}}^{t_{i+2}}\int_{2Q}|\nabla e^{-t^2L^s}\phi_s|^2dxdt
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-1}}^{t_{i+2}}\int_{\frac{5}{4}Q} |\nabla \partial_t e^{-t^2L^s}\phi_s|^2dxdt
    \\
    &\qquad+ \frac{1}{s^2}\int_{t_{i-1}}^{t_{i+2}}\int_{\frac{5}{4}Q} |\partial_k v(x,k,s)|^2 dxdk
\end{align*}
Further, we will have to apply \reflemma{lemma:LEMMA5}. Hence we have to introduce the smooth cut-off function \(\eta\) and choose \(\frac{5}{4}\leq\EPS_1<\EPS_2\leq\frac{3}{2}\), \(d:=(\EPS_2-\EPS_1)/2\), i.e. \(\eta\equiv 1\) on \(\EPS_1 Q\times[\frac{1}{\EPS_1}t_{i-1},\EPS_1t_{i+2}]\) and \(\eta\equiv 0\) on \(\Omega\setminus (\EPS_2 Q\times [\frac{1}{\EPS_2}t_{i-2},\EPS_2 t_{i+3}])\) with \(|\nabla \eta|\lesssim \frac{1}{ds}\), where we set
\begin{align*}
&Q^*:=\EPS_1 Q\times[\frac{1}{\EPS_1}t_{i-1},\EPS_1t_{i+2}],\qquad \tilde{Q}^*:=(\EPS_1+d) Q\times[\frac{1}{\EPS_1+d}t_{i-1},(\EPS_1+d)t_{i+2}], 
\\
&\hat{Q}^*:=\EPS_2 Q\times[\frac{1}{\EPS_2}t_{i-1},\EPS_2t_{i+2}].
\end{align*}

Then we have

\begin{align*}
    &\int_{Q^*}|\partial_k v(x,k,s)|^2dkdx=\int_{\tilde{Q}^*}\int_{\EPS_2 Q}\partial_k v\big(2kL^s v + k\Div(\partial_s A\nabla e^{-k^2L^s}\phi_s)\big)\eta^2 dkdx 
    \\
    &\qquad=\int_{\tilde{Q}^*}\nabla \partial_k v \nabla v\eta^2kdxdk + \int_{\tilde{Q}^*}\nabla \partial_k v \partial_s A\nabla e^{-k^2L^s}\phi_s\eta^2kdxdk
    \\
    &\qquad\quad + \int_{\tilde{Q}^*} \partial_k v \nabla v\nabla\eta^2kdxdk + \int_{\tilde{Q}^*} \partial_k v \partial_s A\nabla e^{-k^2L^s}\phi_s\nabla\eta^2kdxdk
    \\
    &\qquad=: II_1+II_2+II_3+II_4.
\end{align*}
We estimate each integral separately using the same techniques consisting of Hölder's inequality, \reflemma{Lemma:CacciopolliTypeInequalities}, \reflemma{lemma:UnifromBoundOnrholocally} and hiding of terms on the left hand side. At this point, we will be more precise and show these calculations for all terms. First, for \(II_1\)
\begin{align*}
    II_1&\lesssim s\Big(\int_{\tilde{Q}^*}|\nabla v|^2dxdk\Big)^{1/2}\Big(\int_{\tilde{Q}^*}|\nabla\partial_k v|^2dxdk\Big)^{1/2}
    \\
    &\lesssim s\Big(\frac{1}{d^2s^2}\int_{\hat{Q}^*}|v(x,k,s)|^2dxdk + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk\Big)^{1/2}
    \\
    &\quad\cdot \Big(\frac{1}{d^2s^2}\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^2s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk\Big)^{1/2}
    \\
    &\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^4s^2}\int_{\tilde{Q}^*}|v(x,k,s)|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
\end{align*}

Furthermore, we have
\begin{align*}
    II_2&\lesssim \sigma d^2s^2\int_{\tilde{Q}^*}|\nabla \partial_k v|^2dxdk + \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\tilde{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \big(\frac{1}{d^2}+1\big)\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}
and
\begin{align*}
    II_3&\lesssim \sigma \int_{\tilde{Q}^*}|\partial_k v|^2dxdk + \frac{C_\sigma}{d^2}\int_{\tilde{Q}^*}|\nabla v|^2dxdk
    \\
    &\lesssim \sigma \int_{\hat{Q}^*}|\partial_k v|^2dxdk + \frac{1}{d^4s^2}\int_{\hat{Q}^*}\int_{2Q}|v(x,k,s)|^2dxdk
    \\
    &\qquad+ \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}
and
\begin{align*}
    II_4\lesssim \sigma \int_{\tilde{Q}^*}|\partial_k v|^2dxdk + \frac{1}{d^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\tilde{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk.
\end{align*}

Putting all these integrals together we obtain 
\begin{align*}
    \int_{\tilde{Q}^*}|\partial_k v|^2dxdk&\lesssim \sigma\int_{\hat{Q}^*}|\partial_k v(x,k,s)|^2dxdk + \frac{1}{d^4s^2}\int_{\tilde{Q}^*}|v(x,k,s)|^2dxdk
    \\
    &\qquad + \big(1+\frac{1}{d^2}\big)\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{\hat{Q}^*}|\nabla e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 d^2s^2 \int_{\hat{Q}^*}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
\end{align*}

which leads with \reflemma{lemma:LEMMA5} to
\begin{align*}
    I_2&\lesssim\frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_k e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{\frac{5}{4}Q} |\nabla \partial_k e^{-k^2L^s}\phi_s|^2dxdk
    \\
    &\qquad+ \frac{1}{s^2}\int_{t_{i-2}}^{t_{i+3}}\int_{\frac{5}{4}Q} |\partial_k v(x,k,s)|^2 dxdk
    \\
    &\lesssim \frac{1}{s^4}\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad + \frac{1}{s^2}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk,
\end{align*}

and hence
\begin{align*}
    \int_Q |\nabla w_s^{(2)}(x,s)|^2dx&=I_1+sI_2
    \\
    &\lesssim \frac{1}{s^3}\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad + \frac{1}{s}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad+  s\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk.
\end{align*}




Now, we can show the global estimates \eqref{lemma:Nablaw_s^2SpatialBound} and \eqref{lemma:w_s^2SqFctBound2}. We use above introduced partition of \((t_j)_j\) and set \(\mathcal{D}_j\) as the collection of a decomposition of \(3\Delta\) into cubes \(Q\) of size \(l(Q)\approx t_j\). First for \eqref{lemma:Nablaw_s^2SpatialBound} we have for \(s\approx t_i\)
\begin{align*}
    &\int_{\mathbb{R}^n} |\nabla w_s^{(2)}(x,s)|^2 sdxds\leq \sum_{Q\in \mathcal{D}_j} |\nabla w_s^{(2)}(x,s)|^2 sdxds
    \\
    &\qquad\lesssim \sum_{Q\in \mathcal{D}_j}\Big(\frac{1}{s^2}\fint_{t_{i-3}}^{t_{i+4}}\int_{2Q}|v(x,k,s)|^2dkdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad\qquad+  s^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk\Big)
    \\
    &\qquad\lesssim \frac{1}{s^2}\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|v(x,k,s)|^2dkdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n} |\nabla e^{-k^2L^s}\phi_s|^2dxdk 
    \\
    &\qquad\qquad+  s^2\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|\nabla\partial_ke^{-k^2L^s}\phi_s|^2dxdk\Big).
\end{align*}

We note here that due to \reflemma{lemma:nablaSemigroupBoundedByNablaf} and \eqref{equation:L2ofnablaphiBounded}
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-2}}^{t_{i+3}}\int_{\mathbb{R}^n}|\nabla e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|,\]
and
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \fint_{t_{i-3}}^{t_{i+4}}\int_{\mathbb{R}^n}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|.\]

Since we can also proof 
\[\int_{\mathbb{R}^n}|v(x,t,s)|^2dx\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s^2 \]
analogously to the proof of \eqref{lemma:w_s^2spatialL^2Bound} in \reflemma{lemma:w_s^2/nablaw_s^2spatialL^2Bound}, we obtain 

\begin{align*}
    \int_{3\Delta} |\nabla w_s^{(2)}(x,s)|^2 sdxds\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2|\Delta|,
\end{align*}
which yields \eqref{lemma:Nablaw_s^2SpatialBound}. At last, \eqref{lemma:w_s^2SqFctBound2} is direct consequence of \eqref{lemma:Nablaw_s^2SpatialBound}. To see this we note with \eqref{condition:L^2Carlesontypecond} 
\begin{align*}
    \int_0^\infty \int_{\mathbb{R}^n} |\nabla w_s^{(2)}(x,s)|^2 sdxds \lesssim |\Delta|\int_0^\infty \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}^2s ds.
\end{align*}





Then
\begin{align*}
    \int_{3\Delta}\int_0^\infty |\nabla w_s^{(2)}(x,s)|^2 sdxds\leq \sum_{j, Q\in \mathcal{D}_j}\int_Q\int_{t_i}^{t_{i+1}} |\nabla w_s^{(2)}(x,s)|^2 sdxds.
\end{align*}
We can apply the local estimate (\ref{lemma:localEstimateNablaw_s^2}) to obtain
\begin{align*}
    &\sum_{j, Q\in \mathcal{D}_j}\int_Q\int_{t_i}^{t_{i+1}} |\nabla w_s^{(2)}(x,s)|^2 sdxds
    \\
    &\lesssim \sum_{j, Q\in \mathcal{D}_j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{Q}|v(x,t,s)|^2dtdx
    \\
    &\qquad \qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{2Q} |\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{Q}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds
    \\
    &\lesssim \sum_{j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|v(x,t,s)|^2dtdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta} |\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds.
\end{align*}
We note here that due to \reflemma{lemma:nablaSemigroupBoundedByNablaf} and (\ref{equation:L2ofnablaphiBounded})
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|\nabla e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|,\]
and
\[\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \fint_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdk\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|.\]

Since we can also proof 
\[\int_{3\Delta}|v(x,t,s)|^2dx\lesssim \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s^2 \]
analogously to the proof of \ref{lemma:w_s^2spatialL^2Bound} in \reflemma{lemma:w_s^2/nablaw_s^2spatialL^2Bound}, we get in total

\begin{align*}
    &\sum_{j}\int_{t_i}^{t_{i+1}}\Big(\frac{1}{t_i^2}\int_{t_{i-2}}^{t_{i+3}}\int_{3\Delta}|v(x,t,s)|^2dtdx
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla e^{-t^2L^s}\phi_s|^2dxdt  
    \\
    &\qquad \qquad+ \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 s^2 \int_{t_{i-3}}^{t_{i+4}}\int_{3\Delta}|\nabla\partial_t e^{-t^2L^s}\phi_s|^2dxdt\Big)ds.
    \\
    &\lesssim \sum_j\int_{t_i}^{t_{i+1}} \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s ds= \int_0^\infty \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2|\Delta|s ds.
\end{align*}










\end{proof}
\end{comment}

















\subsection{The partial derivative part \(w_t\)}


\begin{lemma}\label{lemma:SqFctBoundsForw_t}
If we assume \eqref{condition:L^1Carlesontypecond}, the following square function bounds involving \(w_t\) hold
\begin{enumerate}[(1)]
    \item \[\Big\Vert\Big(\int_0^\infty\frac{|w_t|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}=\Big\Vert\Big(\int_0^\infty\frac{|sL^se^{-\eta^2s^2L^s}\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|,\]\label{lemma:w_tSqFctBound1}
    \item \[\Big\Vert\Big(\int_0^\infty\frac{|s\nabla w_t|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|,\label{lemma:w_tSqFctBound2}\]
    \item \[\Big\Vert\Big(\int_0^\infty\frac{|s^2L^sw_t|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}\lesssim |\Delta|.\label{lemma:w_tSqFctBound3}\]
\end{enumerate}
\end{lemma}

\begin{proof}
We start with proving \eqref{lemma:w_tSqFctBound1}. First, set \(f_{s^2}:=(L^s)^{1/2}\phi^s\) and use the substitution \(\tau=s^2\) to obtain
\begin{align*}
    \Big\Vert\Big(\int_0^\infty\frac{|sL^se^{-\eta^2s^2L^s}\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}&=\Big\Vert\Big(\int_0^\infty|(L^{\sqrt{\tau}})^{1/2}e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau|^2d\tau\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}|(L^{\sqrt{\tau}})^{1/2}e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau|^2 dxd\tau
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}|\nabla e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau|^2 dxd\tau.
\end{align*}
Here we used the Kato Conjecture \refprop{prop:KatoConjecture} in the last step. Next, we can use ellipticity and integration by parts to get
\begin{align*}
    &\int_0^\infty\int_{\mathbb{R}^n}A(x,\sqrt{\tau})\nabla e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau(x) \cdot \nabla e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau(x)  dx d\tau
    \\
    &\qquad =\int_0^\infty\int_{\mathbb{R}^n}L^{\sqrt{\tau}}e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau dx d\tau.
\end{align*}
Analogously to how we calculated the partial derivative \(\partial_s w\) we can now handle \(\partial_\tau e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\) and see that

\begin{align*}
&\int_0^\infty\int_{\mathbb{R}^n}L^{\sqrt{\tau}}e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau dx d\tau
\\
&\quad=\int_0^\infty\int_{\mathbb{R}^n}\partial_\tau e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau dxd\tau 
\\
&\qquad-\int_0^\infty\int_{\mathbb{R}^n}\frac{1}{\sqrt{\tau}}\Big(\int_0^{\eta^2\tau} e^{-(\eta^2\tau-r)L^{\sqrt{\tau}}}\Div(\partial_t A(x,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau) dr
\\
&\qquad\qquad\qquad\qquad\qquad- e^{-\eta^2\tau L^{\sqrt{\tau}}}\partial_\tau f_\tau \Big)e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau dxd\tau
\\
&\quad=\int_0^\infty -\frac{1}{2}\frac{d}{d \tau}\Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2^2 d\tau
\\
&\qquad+\int_0^\infty \frac{1}{\sqrt{\tau}}\int_0^{\eta^2\tau} \Vert e^{-(\eta^2\tau-r)L^{\sqrt{\tau}}}\Div(\partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau)\Vert_2 
\\
&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\cdot\Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2 dr d\tau 
\\
&\qquad+\int_0^\infty \frac{1}{\sqrt{\tau}} \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}\partial_\tau f_\tau\Vert_2 \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2 d\tau.
\end{align*}

Let us consider the terms separately. First, we note by \refprop{prop:L2NormGoesTo0} 
\begin{align*}
\int_0^\infty -\frac{1}{2}\frac{d}{d \tau}\Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2^2 d\tau&=\lim_{\tau\downarrow 0}\Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2^2+\lim_{\tau\uparrow \infty}\Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2^2
\\
&\lesssim\lim_{\tau\downarrow 0}\Vert f_\tau\Vert_2^2.
\end{align*}
By the Kato Conjecture \refprop{prop:KatoConjecture} and the definition of \(f_\tau\) we get
\[\Vert f_\tau\Vert_2^2\lesssim \Vert \nabla \phi^{\sqrt{s}}\Vert_2^2\lesssim |\Delta|,\]
and hence that the first term is bounded by \(|\Delta|\).

For the next term, we evaluate by dualising and integration by parts
\begin{align*}
    &\Vert e^{-(\eta^2\tau-r)L^{\sqrt{\tau}}}\Div(\partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau)\Vert_2
    \\
    &\qquad =\sup_{h\in L^2(\mathbb{R}^n), \Vert h\Vert_2=1}\int_{\mathbb{R}^n} e^{-(\eta^2\tau-r)L^{\sqrt{\tau}}}\Div(\partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau) h dx
    \\
    &\qquad =\sup_{h\in L^2(\mathbb{R}^n), \Vert h\Vert_2=1}\int_{\mathbb{R}^n} \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau \cdot\nabla e^{-(\eta^2\tau-r)(L^{\sqrt{\tau}})^*}h dx
    \\
    &\qquad \leq \sup_{h\in L^2(\mathbb{R}^n), \Vert h\Vert_2=1}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty \Vert\nabla e^{-r L^{\sqrt{\tau}}}f_\tau\Vert_2\Vert\nabla e^{-(\eta^2\tau-r)(L^{\sqrt{\tau}})^*}h\Vert_2
    \\
    &\qquad \lesssim \sup_{h\in L^2(\mathbb{R}^n), \Vert h\Vert_2=1}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty \frac{1}{\sqrt{r}\sqrt{\eta^2\tau-r}}\Vert f_\tau\Vert_2\Vert h\Vert_2.
\end{align*}
In the last line we used \refprop{prop:L2NormBoundsOfHeatSemigroup}. Since \(\Vert f_\tau\Vert_2\lesssim |\Delta|^{1/2}\) we get in total for the second term
\begin{align*}
    &\int_0^\infty \frac{1}{\sqrt{\tau}}\int_0^{\eta^2\tau} \Vert e^{-(\eta^2\tau-r)L^{\sqrt{\tau}}}\Div(\partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\nabla e^{-r L^{\sqrt{\tau}}}f_\tau)\Vert_2 \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2 dr d\tau 
    \\
    &\qquad\lesssim \int_0^\infty \frac{1}{\sqrt{\tau}}\int_0^{\eta^2\tau}  \frac{1}{\sqrt{r}\sqrt{\eta^2\tau-r}}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty|\Delta|^{1/2} \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2 dr d\tau 
    \\
    &\qquad\lesssim \int_0^\infty \frac{1}{\sqrt{\tau}}\int_0^{\eta^2\tau}  \frac{1}{\sqrt{r}\sqrt{\eta^2\tau-r}}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty|\Delta|^{1/2} \Vert f_\tau\Vert_2 dr d\tau
    \\
    &\qquad\lesssim \int_0^\infty \frac{1}{\sqrt{\tau}}\int_0^{\eta^2\tau}  \frac{1}{\sqrt{r}\sqrt{\eta^2\tau-r}}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty |\Delta| dr d\tau
    \\
    &\qquad\lesssim \int_0^\infty \frac{1}{\sqrt{\tau}}\Vert \partial_t A(\cdot,t)|_{t=\sqrt{\tau}}\Vert_\infty |\Delta| d\tau.
\end{align*}
Using the substitution \(s^2=\tau\) we get
\[\int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty |\Delta|ds.\]

Finally for the last term we have
\begin{align*}
    \int_0^\infty \frac{1}{\sqrt{\tau}} \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}\partial_\tau f_\tau\Vert_2 \Vert e^{-\eta^2\tau L^{\sqrt{\tau}}}f_\tau\Vert_2 d\tau &\lesssim \int_0^\infty \frac{1}{\sqrt{\tau}} \Vert \partial_\tau f_\tau\Vert_2 \Vert f_\tau\Vert_2 d\tau
    \\
    &\lesssim \int_0^\infty\Vert \partial_s f_{s^2}\Vert_2|\Delta|^{1/2}ds 
    \\
    &\lesssim \int_0^\infty\Vert \partial_s \nabla\phi^s\Vert_2|\Delta|^{1/2}ds
    \\
    &\lesssim \int_0^\infty\Vert\partial_s A(\cdot,s)\Vert_\infty |\Delta|ds.
\end{align*}
The last line follows by \eqref{equation:L2ofpartial_snablaphiBounded} and finishes the proof of \eqref{lemma:w_tSqFctBound1}.

\hfill\\
The proofs of \eqref{lemma:w_tSqFctBound2} and \eqref{lemma:w_tSqFctBound3} rely on \eqref{lemma:w_tSqFctBound1} and \refprop{prop:L2NormBoundsOfHeatSemigroup}. For \eqref{lemma:w_tSqFctBound2} we see that
\begin{align*}
    &\Big\Vert\Big(\int_0^\infty\frac{|s^2\nabla L^s e^{-\eta^2s^2L^s}\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}\frac{|s^2\nabla L^s e^{-\eta^2s^2L^s}\phi^s|^2}{s} dxds
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}\frac{|s\nabla e^{-\frac{\eta^2s^2}{2}L^s}(sL^s e^{-\frac{\eta^2s^2}{2}L^s}\phi^s)|^2}{s} dxds
    \\
    &\lesssim \int_0^\infty\int_{\mathbb{R}^n}\frac{|s L^s e^{-\frac{\eta^2s^2}{2}L^s}\phi^s|^2}{s} dxds,
\end{align*}
where the last integral is bounded by \eqref{lemma:w_tSqFctBound1}. Similar we observe for \eqref{lemma:w_tSqFctBound3}
\begin{align*}
    &\Big\Vert\Big(\int_0^\infty\frac{|s^2L^s L^s e^{-\eta^2s^2L^s}\phi^s|^2}{s}ds\Big)^{1/2}\Big\Vert_{L^2(\mathbb{R}^n)}
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}\frac{|s^2 L^s L^s e^{-\eta^2s^2L^s}\phi^s|^2}{s} dxds
    \\
    &=\int_0^\infty\int_{\mathbb{R}^n}\frac{|s L^s e^{-\frac{\eta^2s^2}{2}L^s}(sL^s e^{-\frac{\eta^2s^2}{2}L^s}\phi^s)|^2}{s} dxds
    \\
    &\lesssim \int_0^\infty\int_{\mathbb{R}^n}\frac{|s L^s e^{-\frac{\eta^2s^2}{2}L^s}\phi^s|^2}{s} dxds.
\end{align*}

\end{proof}


In contrast to \(\partial_s\phi^s-w_s^{(1)}\) and \(w_s^{(2)}\) we have a certain local Harnack-type property for \(w_t\). First we have 

\begin{prop}[Proposition 6 in \cite{hofmann_dirichlet_2022}]\label{prop:Proposition6}
    Let \(L\) be a t-independent operator, \(Q\subset\mathbb{R}^n\) be a cube with side length \(l(Q)=R_0\) and \(\hat{Q}:=(1+\varepsilon)Q\) be an enlarged cube for some fixed \(\frac{1}{2}>\varepsilon>0\). Then
    \[\sup_{Q\times (R_0,2R_0]}|\partial_t e^{-t^2L}f(x)|^2\lesssim \fint_{\hat{Q}}\int_{(1-\varepsilon)R_0}^{2(1+\varepsilon)R_0}\frac{|\partial_t e^{-t^2L}f(x)|^2}{t}dxdt.\]
\end{prop}

This result is used to proof the extension to our case where we do have a operator family that depend on t, which is the following result.

\begin{lemma}\label{lemma:localHarnackTypeInequalityForw_t}
    Fix a boundary cube \(\Delta\). Then with the notation of \refprop{prop:Proposition6}
    \begin{align*}
    \sum_{k\leq k_0}\sum_{Q\in \mathcal{D}_k(\Delta)}|Q|\sup_{Q\times (2^{-k},2^{-k+1}]}|w_t|^2&\lesssim \sum_{k\leq k_0}\sum_{Q\in \mathcal{D}_k(\Delta)}\int_{\hat{Q}}\int_{(1-\varepsilon)2^{-k}}^{(1+\varepsilon)2^{-k+1}}\frac{|w_t(x,s)|^2}{s}dxds
    \\
    &\qquad + |\Delta|\int_0^{l(\Delta)}\Vert\partial_s A(\cdot,s)\Vert_\infty^2 s ds.
    \end{align*}
\end{lemma}

\begin{proof}
The first step of the proof is to apply \refprop{prop:Proposition6} for every operator \(L^s\) with \(s\in [R_0,2R_0]\), where \(R_0=2^{-k}\), to get
\begin{align*}
    \sup_{(x,s)\in Q\times [R_0,2R_0]}|w_t(x,s)|&\lesssim \sup_{s\in [R_0,2R_0]}\fint_{\hat{Q}}\int_{(1-\varepsilon)R_0}^{2(1+\varepsilon)R_0}\frac{|\partial_t w(x,t^2,s)|^2}{t}dxdt
    \\
    &=\fint_{\hat{Q}}\int_{R_0}^{2R_0}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}dxdt,
\end{align*}    
where \(s^*\) is the value of s where the supremum is attained. Let \(\psi\in C^\infty(\Omega)\) be a smooth cuf-off function, i.e. 
\[\psi\equiv 1 \textrm{ on } (1+\EPS_1)\hat{Q}\times [(1-\EPS_1)R_0,2(1+\EPS_1)R_0],\]
and
\[\psi\equiv 0 \textrm{ on } \Omega\setminus (1+\EPS_1+d)Q\times [(1-2\EPS_1-d)R_0,2(1+\EPS_1+d)R_0],\]
and
\[\Vert \nabla \psi \Vert \lesssim_\epsilon \frac{1}{d R_0}\]
for some fixed sufficiently small \(\epsilon>0\) and \(0<\EPS_1<\EPS_2<\EPS\) with \(d:=(\EPS_2-\EPS_1)/3\). Define the enlargements
\[\tilde{Q}:=(1+\EPS_1+2d)Q\qquad\textrm{and}\qquad \bar{Q}:=(1+\EPS_1+3d)Q,\]
and
\begin{align*}
&\tilde{Q}^*:=\tilde{Q}\times[(1-\EPS_1-2d)R_0,2(1+\EPS_1+2d)R_0],
\\
\textrm{and}\quad &\bar{Q}^*:=\bar{Q}\times[(1-\EPS_1-3d)R_0,2(1+\EPS_1+3d)R_0].
\end{align*}
Furthermore, let us calculate \(\partial_s\partial_t w(x,t^2,s)\), which is
\begin{align*}
    \partial_s\partial_t w(x,t^2,s)&=\partial_s (2tL^sw(x,t^2,s))
    \\
    &=2t\Div(\partial_s\AP(x,s)\nabla w(x,t^2,s))+2tL^s\partial_sw(x,t^2,s)
    \\
    &=2t\Div(\partial_s\AP(x,s)\nabla w(x,t^2,s))
    \\
    &\qquad + 2tL^sv_1(x,t^2,s)+2tL^sv_2(x,t^2,s).
\end{align*}

Thus, we obtain
\begin{align*}
    &\fint_{\hat{Q}}\int_{(1-\EPS_1-d)R_0}^{2(1+\EPS_1+d)R_0}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}dxdt
    \\
    &\leq \fint_{\tilde{Q}}\int_{(1-\EPS_1-2d)R_0}^{2(1+\EPS_1+2d)R_0}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}\psi(x,t) dxdt
    \\
    &= \fint_{\tilde{Q}^*}\partial_t w(x,t^2,s^*)\Big(\partial_t w(x,t^2,t) + \int_t^{s^*}\partial_s\partial_t w(x,t^2,s)ds\Big)\psi(x,t) dxdt
    \\
    &= \fint_{\tilde{Q}^*}\partial_t w(x,t^2,s^*)\partial_t w(x,t^2,t)\psi(x,t) dxdt
    \\
    &\qquad+2\fint_{\tilde{Q}^*}\int_t^{s^*}\partial_t w(x,t^2,s^*)t\Div(\partial_s\AP(x,s)\nabla w(x,t^2,s))\psi(x,t) dsdxdt
    \\
    &\qquad +2\fint_{\tilde{Q}^*}\int_t^{s^*}\partial_t w(x,t^2,s^*)tL^sv_1(x,t^2,s)\psi(x,t) dsdxdt
    \\
    &\qquad+2\fint_{\tilde{Q}^*}\int_t^{s^*}\partial_t w(x,t^2,s^*)tL^sv_2(x,t^2,s)\psi(x,t) dsdxdt
    \\
    &=:I_1+I_2+I_3+I_4.
\end{align*}
First, let us consider \(I_1\). We have
\begin{align*}
    I_1&\lesssim \sigma \frac{1}{|Q|}\int_{\tilde{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{t} dxdt +C_\sigma\frac{1}{|Q|}\int_{\tilde{Q}^*}\frac{|\partial_t w(x,t^2,t)|^2}{t} dxdt.
\end{align*}

For \(I_2\) we use integration by parts to get
\begin{align*}
    I_2&=\fint_{\tilde{Q}^*}\int_t^{s^*}\partial_t \nabla w(x,t^2,s^*)\psi(x,t)\partial_s\AP(x,s)\nabla w(x,t^2,s) tdsdxdt
    \\
    &\qquad+\fint_{\tilde{Q}^*}\int_t^{s^*} \nabla\psi(x,t) \partial_t w(x,t^2,s^*)\partial_s\AP(x,s)\nabla w(x,t^2,s) tdsdxdt
    \\
    &\lesssim\fint_{\tilde{Q}^*}\int_t^{s^*}|\partial_t \nabla w(x,t^2,s^*)||\partial_s\AP(x,s)||\nabla w(x,t^2,s)| tdsdxdt
    \\
    &\qquad+\fint_{\tilde{Q}^*}\int_t^{s^*} \frac{|\partial_t w(x,t^2,s^*)|}{d t}|\partial_s\AP(x,s)||\nabla w(x,t^2,s)| tdsdxdt
    \\
    &\lesssim \int_{(1-\EPS_1+2d)R_0}^{2(1+\EPS_1+2d)R_0}\Big(\fint_{\tilde{Q}}|\partial_t \nabla w(x,t^2,s^*)|^2dxdt\Big)^\frac{1}{2}\Vert \partial_s\AP(\cdot,s)\Vert_\infty \Big(\fint_{\tilde{Q}}|\nabla w(x,t^2,s)|^2dxdt\Big)^\frac{1}{2}sds
    \\
    &\qquad +\int_{(1-\EPS_1-2d)R_0}^{2(1+\EPS_1+2d)R_0}\Big(\fint_{\tilde{Q}}\frac{|\partial_t w(x,t^2,s^*)|^2}{d^2t^2}dxdt\Big)^\frac{1}{2}\Vert \partial_s\AP(\cdot,s)\Vert_\infty \Big(\fint_{\tilde{Q}}|\nabla w(x,t^2,s)|^2dxdt\Big)^\frac{1}{2}sds
\end{align*}

Since we have a Cacciopolli inequality for \(\partial_t w\) (see Remark \ref{remark:CaccForpartial_tw}) we obtain
\[\fint_{\tilde{Q}}|\partial_t \nabla w(x,t^2,s^*)|^2dxdt\lesssim\fint_{\bar{Q}}\frac{|\partial_t w(x,t^2,s^*)|^2}{d^2t^2}dxdt,\]
and due to \refprop{Proposition11} and \reflemma{lemma:UniformBoundOnM[nablaphi^s]}
\[\fint_{\tilde{Q}}|\nabla w(x,t^2,s)|^2dxdt\lesssim \kappa_0.\]
Together this gives
\[I_2\lesssim \sigma \frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{t} dxdt +\frac{1}{d^2} \int_{(1+2\varepsilon)R_0}^{2(1+2\varepsilon)R_0}\Vert \partial_s\AP(\cdot,s)\Vert_\infty^2 s ds.\]

The integral \(I_3\) and \(I_4\) can be handled similarly. 

First for \(I_3\), we use integration by parts to obtain
\begin{align*}
    I_3&=\fint_{\tilde{Q}^*}\int_t^{s^*}\partial_t \nabla w(x,t^2,s^*)\psi(x,t)A(x,s)\nabla v_1(x,t^2,s) sdsdxdt
    \\
    &\qquad+\fint_{\tilde{Q}^*}\int_t^{s^*} \nabla\psi(x,t) \partial_t w(x,t^2,s^*) A(x,s)\nabla v_1(x,t^2,s) sdsdxdt
    \\
    &\lesssim\fint_{\tilde{Q}^*}\int_t^{s^*}|\partial_t \nabla w(x,t^2,s^*)||\nabla v_1(x,t^2,s)| sdsdxdt
    \\
    &\qquad+\fint_{\tilde{Q}^*}\int_t^{s^*} \frac{|\partial_t w(x,t^2,s^*)|}{dt}|\nabla v_1(x,t^2,s)| sdsdxdt
    \\
    &\lesssim \int_{(1-\EPS_1-2d)R_0}^{2(1+\EPS_1+2d)R_0}\Big(\fint_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{d^2t^2}dxdt\Big)^\frac{1}{2} \Big(\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2dxdt\Big)^\frac{1}{2}sds
\end{align*}

We arrive at
\[I_3\lesssim \sigma \frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{t} dxdt + \frac{1}{d^2}\int_{(1-\EPS_1-2d)R_0}^{2(1+\EPS_1 +2d)R_0}\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2sdxdtds.\]

Completely analogously for \(I_4\), we arrive at
\[I_4\lesssim \sigma \frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{t} dxdt + \frac{1}{d^2}\int_{(1-\EPS_1-2d)R_0}^{2(1+\EPS_1+2d)R_0}\fint_{\tilde{Q}^*}|\nabla v_2(x,t^2,s)|^2sdxdtds.\]

Thus, we can put all pieces together to get
\begin{align*}
    \fint_Q\int_{(1-\EPS_1)R_0}^{2(1+\EPS_1)R_0}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}dxdt
    &\lesssim \sigma \frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}dxdt 
    \\
    &\qquad +\frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,t)|^2}{t} 
    \\
    &\qquad +\frac{1}{d^2} \int_{(1-3\varepsilon)R_0}^{2(1+3\varepsilon)R_0}\Vert \partial_s A(\cdot,s)\Vert_\infty^2 s ds
    \\
    &\qquad +\frac{1}{d^2} \int_{(1-3\varepsilon)R_0}^{2(1+3\varepsilon)R_0}\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2sdxdtds 
    \\
    &\qquad + \frac{1}{d^2}\int_{(1-3\varepsilon)R_0}^{2(1+3\varepsilon)R_0}\fint_{\tilde{Q}^*}|\nabla v_2(x,t^2,s)|^2sdxdtds
\end{align*}

Applying  \reflemma{lemma:LEMMA5} we get
\begin{align*}
    \fint_{\hat{Q}}\int_{R_0}^{2R_0}\frac{|\partial_t w(x,t^2,s^*)|^2}{t}dxdt
    &\lesssim \frac{1}{|Q|}\int_{\bar{Q}^*}\frac{|\partial_t w(x,t^2,t)|^2}{t}dxdt 
    \\
    &\qquad + \int_{(1-3\varepsilon)R_0}^{2(1+3\varepsilon)R_0}\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2sdxdtds 
    \\
    &\qquad + \int_{(1-3\varepsilon)R_0}^{2(1+3\varepsilon)R_0}\fint_{\tilde{Q}^*}|\nabla v_2(x,t^2,s)|^2sdxdtds
\end{align*}






If we combine the Cacciopolli type inequality in \reflemma{Lemma:CacciopolliTypeInequalities} with the observation that the proof of \eqref{lemma:w_s^2spatialL^2Bound} in \reflemma{lemma:w_s^2/nablaw_s^2spatialL^2Bound} does also work for \(v_1(x,t^2,s)\) instead of just \(w_s^{(2)}(x,s)=v_1(x,s^2,s)\), we can estimate 
\begin{align*}
    &\sum_{Q\in \mathcal{D}_k}|Q|\int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2 sdxdtds
    \\
    &\lesssim \sum_{Q\in \mathcal{D}_k}|Q|\int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\fint_{\tilde{Q}^*}|\nabla v_1(x,t^2,s)|^2 s dxdt ds
    \\
    &\lesssim \sum_{Q\in \mathcal{D}_k}|Q|\int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Big(\frac{1}{s}\fint_{2Q^*}|v(x,t,s)|^2dxdt 
    \\
    &\qquad\qquad + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2\int_{t_{i-1}}^{t_{i+2}}\fint_{2Q}|\nabla e^{-k^2L^s}\phi_s|^2dkdx  \Big)ds
    \\
    &\lesssim \int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Big(\fint_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\frac{1}{s}\int_{3\Delta} |v(x,t,s)|^2 dx dt \Big)
    \\
    &\qquad\qquad + \Big(\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-1}}^{t_{i+2}}\int_{3\Delta}|\nabla e^{-k^2L^s}\phi_s|^2dkdx\Big) ds
\end{align*}
Using \reflemma{lemma:nablaSemigroupBoundedByNablaf} and \eqref{equation:L2ofnablaphiBounded} we observe
\[\int_{3\Delta}|\nabla e^{-k^2L^s}\phi_s|^2dx\lesssim |\Delta|,\]
and hence
\begin{align*}
    &\int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Big(\fint_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\frac{1}{s}\int_{3\Delta} |v(x,t,s)|^2 dx dt \Big)
    \\
    &\qquad\qquad + \Big(\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 \int_{t_{i-1}}^{t_{i+2}}\int_{3\Delta}|\nabla e^{-k^2L^s}\phi_s|^2dkdx\Big) ds
    \\
    &\lesssim \int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Big(\fint_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\frac{1}{s}\int_{3\Delta} |v(x,t,s)|^2 dx dt \Big) + \Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 |\Delta| s ds
    \\
    &\lesssim \int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 |\Delta| s ds.
\end{align*}
Similarly, we can see with \reflemma{lemma:nablaSemigroupBoundedByNablaf} and \eqref{equation:L2ofpartial_snablaphiBounded} that
\[\Vert \nabla v_2(\cdot,t,s)\Vert_{L^2(\mathbb{R}^n)}\lesssim \Vert \partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}|\Delta|^{1/2},\]
and hence
\begin{align*}
    &\sum_{Q\in \mathcal{D}_k}|Q|\int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\fint_{\tilde{Q}^*}|\nabla v_2(x,t^2,s)|^2 sdxdtds
    \\
    &\lesssim \int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\fint_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\int_{3\Delta}|\nabla v_2(x,t^2,s)|^2 sdxdtds
    \\
    &\lesssim \int_{(1-3\EPS)R_0}^{2(1+3\EPS)R_0}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(3\Delta)}^2 |\Delta| s ds.
\end{align*}

Thus,
\begin{align*}
    \sum_{k\leq k_0}\sum_{Q\in \mathcal{D}_k(\Delta)}|Q|\sup_{Q\times (2^{-k},2^{-k+1}]}|w_t|&\lesssim \sum_{k\leq k_0}\sum_{Q\in \mathcal{D}_k(\Delta)}\int_{\bar{Q}^*}\frac{|w_t(x,s)|^2}{s}dxds
    \\
    &\qquad + |\Delta|\int_0^{l(\Delta)}\Vert\partial_s A(\cdot,s)\Vert_\infty^2 s ds.
\end{align*}


\end{proof}












==> SquareFunctionResults.tex <==
\section{Square function results of the operator \(\mathcal{P}\)}

\subsection{The function \(W_2f\)}
\begin{lemma}
    Let \(f\in C_C(\mathbb{R}^n)\) with \(\mathrm{supp}(f)\subset \Delta\) for a boundary ball \(\Delta\subset\partial\Omega\). Then
    \begin{enumerate}
        \item \(\int_{\Omega}\frac{|W_2f(x,t)|^2}{t}dxdt\lesssim \Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}\)\label{item:GlobalSquareBoundW2}
        \item \(\int_{\Omega}\frac{|t\nabla W_2f(x,t)|^2}{t}dxdt\lesssim \Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}\)\label{item:GlobalSquareBoundNablaW2}
    \end{enumerate}
\end{lemma}

\begin{proof}
    For \eqref{item:GlobalSquareBoundW2} we use Minkowski inequality and (???Kato) to obtain

    \begin{align*}
        &\int_{\Omega}\frac{|W_sf|^2}{s}dxds= \int_0^{\infty}\int_{\mathbb{R}^n}\frac{1}{s}\Big|\int_0^{s} \tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)d\tau\Big|^2 dx ds
        \\
        &\qquad\lesssim \int_0^{\infty}\frac{1}{s}\Big(\int_0^{s}\tau \Vert (L_{||}^s)^{\frac{1}{2}}e^{-(s^2-\tau^2)L_{||}^s}(L_{||}^s)^{-\frac{1}{2}}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L^s_{||}}f)\Vert_{L^2(\mathbb{R}^n)} d\tau\Big)^{2} ds
        \\
        &\qquad\lesssim \int_0^{\infty}\frac{1}{s}\Big(\int_0^{s}\tau \Vert \nabla e^{-(s^2-\tau^2)L_{||}^s}(L_{||}^s)^{-\frac{1}{2}}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L^s_{||}}f)\Vert_{L^2(\mathbb{R}^n)} d\tau\Big)^{2} ds
        \\
        &\qquad\lesssim \int_0^{\infty}\frac{1}{s}\Big(\int_0^{s}\frac{\tau}{\sqrt{s^2-\tau^2}}\Vert(L^s)^{-\frac{1}{2}}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L^s_{||}}f)\Vert_{L^2(\mathbb{R}^n)} d\tau\Big)^2 ds
        \\
        &\qquad\lesssim \int_0^{\infty}\frac{1}{s}\Big(\int_0^{s}\frac{\tau}{\sqrt{s^2-\tau^2}}\Big(\int_{\mathbb{R}^n} |\partial_s A(x,s)\nabla e^{-\tau^2L^s_{||}}f|^2 dx\Big)^{1/2} d\tau\Big)^2 ds
        \\
        &\qquad\lesssim \int_0^{\infty}\frac{1}{s}\Vert\partial_s A(\cdot,s)\Vert_{L^{\infty}(\mathbb{R}^n)}\Big(\int_0^{s}\frac{\tau}{\sqrt{s^2-\tau^2}}\Vert\nabla_{||}f\Vert_{L^2(\mathbb{R}^n)} d\tau\Big)^2 ds
        \\
        &\qquad \lesssim \int_0^\infty \Vert\partial_s A(\cdot,s)\Vert_{L^{\infty}(\mathbb{R}^n)} ds \Vert\nabla_{||}f\Vert_{L^2}^2.
    \end{align*}

    For \eqref{item:GlobalSquareBoundNablaW2} we have by Cacciopolli type inequality (???)
    \begin{align*}
        \int_{\Omega}\frac{|t\nabla W_2f(x,t)|^2}{t}dxdt\lesssim \int_{\Omega}\frac{|W_2f(x,t)|^2}{t}dxdt + \int_0^\infty\Vert\partial_t A(\cdot,t)\Vert_{L^\infty(\mathbb{R}^n)}^2t\Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}^2dxdt\lesssim \Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}
    \end{align*}
\end{proof}

\begin{comment}
\begin{proof}
    \eqref{item:GlobalSquareBoundW2}
    \begin{align*}
        \int_{\Omega}\frac{|W_2f(x,t)|^2}{t}dxdt&=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}\Big(\int_0^t 2\tau e^{-(t^2-t^2)L^t}\mathrm{div}(\partial_t A(x,t)\nabla e^{-\tau^2L^t}f)d\tau\Big) W_2f(x,t)dxdt
        \\
        &=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}\Big(\int_0^t 2\tau\partial_t A(x,t)\nabla e^{-\tau^2L^t}f\cdot \nabla e^{-(t^2-t^2)(L^t)^*}W_2f(x,t) d\tau\Big) dxdt
        \\
        &=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}|\partial_t A(x,t)|\Big(\int_0^t 2\tau|\nabla e^{-\tau^2L^t}f| |\nabla e^{-(t^2-t^2)(L^t)^*}W_2f(x,t)| d\tau\Big) dxdt
        \\
        &\lesssim \Vert\partial_t A\Vert_{\mathcal{C}}\int_{\mathbb{R}^n} \tilde{N}\Big(\fint_0^t 2\tau|\nabla e^{-\tau^2L^t}f| |\nabla e^{-(t^2-t^2)(L^t)^*}W_2f(x,t)| d\tau \Big)dx
    \end{align*}

    Let us look at the expression of the nontangential maximal function. Let \(y\in \partial\Omega\) and \(Q\subset\partial\Omega\) a boundary ball with center in \(y\). Let \(\eta\in C_0^\infty(2Q)\) be a smooth cut-off function with \(\eta\equiv 1\) on \(Q\) and \(|\nabla \eta|\lesssim 1\).
    \begin{align*}
        &\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\fint_0^t 2\tau|\nabla e^{-\tau^2L^t}f| |\nabla e^{-(t^2-t^2)(L^t)^*}W_2f(x,t)| d\tau dt dx
        \\
        &\sum_{k\geq 2}\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}(f\chi_{2^kQ\setminus 2^{k-1}Q})(x)|^2 d\tau dt dx
        \\
        &\qquad + \fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}(f\chi_{2Q})(x)|^2 d\tau dt dx
        \\
        &\sum_{k\geq 2}\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{1}{l(Q)^n}\frac{e^{-c\frac{2^{2k}l(Q)^2}{\tau}}}{\sqrt{t^2-\tau^2}} \Vert f\Vert_{L^2(2^kQ\setminus 2^{k-1}Q)}^2 d\tau dt
        \\
        &\qquad + \fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{1}{l(Q)^n}\frac{1}{\sqrt{t^2-\tau^2}} \Vert f\Vert_{L^2(2Q)}^2 d\tau dt
    \end{align*}

    %======================================




    \eqref{item:GlobalSquareBoundW2}
    \begin{align*}
        \int_{\Omega}\frac{|W_2f(x,t)|^2}{t}dxdt&=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}\Big(\int_0^t 2\tau e^{-(t^2-t^2)L^t}\mathrm{div}(\partial_t A(x,t)\nabla e^{-\tau^2L^t}f)d\tau\Big) W_2f(x,t)dxdt
        \\
        &=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}\Big(\int_0^t 2\tau\partial_t A(x,t)\nabla e^{-\tau^2L^t}f\cdot \nabla e^{-(t^2-t^2)(L^t)^*}W_2f(x,t) d\tau\Big) dxdt
        \\
        &=\int_0^\infty \frac{1}{t}\Big(\int_0^t \Vert 2\tau\partial_t A(x,t)\nabla e^{-\tau^2L^t}f\Vert_{L^2(\mathbb{R}^n)} \Vert\nabla e^{-(t^2-t^2)(L^t)^*}W_2f(\cdot,t)\Vert_{L^2(\mathbb{R}^n)} d\tau\Big) dxdt
        \\
        &\lesssim \int_0^\infty \frac{1}{t}\Big(\int_0^t \frac{1}{\sqrt{t^2-\tau^2}}\Vert 2\tau\partial_t A(x,t)\nabla e^{-\tau^2L^t}f\Vert_{L^2(\mathbb{R}^n)} \Vert W_2f(\cdot,t)\Vert_{L^2(\mathbb{R}^n)} d\tau\Big) dxdt
        \\
        &\lesssim \int_0^\infty \int_{\mathbb{R}^n}\frac{1}{t}|\partial_t A(x,t)|^2\Big(\int_0^t \frac{1}{\sqrt{t^2-\tau^2}} 4\tau^2|\nabla e^{-\tau^2L^t}f|^2d\tau\Big) + \sigma\frac{|W_2f(x,t)|^2}{t}dxdt
    \end{align*}
    For small \(\sigma\) we can hide the last summand on the left hand side and continue for the first one
    \begin{align*}
        &\int_0^\infty \int_{\mathbb{R}^n}\frac{1}{t}|\partial_t A(x,t)|^2\Big(\int_0^t \frac{1}{\sqrt{t^2-\tau^2}} 4\tau^2|\nabla e^{-\tau^2L^t}f|^2d\tau\Big)dxdt
        \\
        &\lesssim \Vert \sup|\partial_tA|^2t\Vert_{\mathcal{C}}\int_{\partial\Omega}\tilde{N}\Big(\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}f|^2 d\tau\Big)d\sigma
    \end{align*}

    
    Let us look at the expression of the nontangential maximal function. Let \(y\in \partial\Omega\) and \(Q\subset\partial\Omega\) a boundary ball with center in \(y\). Let \(\eta\in C_0^\infty(2Q\) be a smooth cut-off function with \(\eta\equiv 1\) on \(Q\) and \(|\nabla \eta|\lesssim 1\), then
    \begin{align*}
        &\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}f(x)|^2\eta^2 d\tau dt dx
        \\
        &=\fint_{2Q}\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} A\nabla e^{-\tau^2L^t}f(x)\cdot\nabla e^{-\tau^2L^t}f(x)\eta^2 d\tau dt dx
        \\
        &=\fint_{2Q}\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau}{\sqrt{t^2-\tau^2}} \partial_te^{-\tau^2L^t}f(x) e^{-\tau^2L^t}f(x)\eta^2 d\tau dt dx
        \\
        &\qquad +\sigma\fint_{2Q}\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}f(x)|^2\eta^2 d\tau dt dx + 
        \\
        &\qquad +C_\sigma\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{1}{\sqrt{t^2-\tau^2}} |e^{-\tau^2L^t}f(x)|^2\eta^2 d\tau dt dx
    \end{align*}

    While the second term can be hidden on the left hand side, we can bound the other two by (???)
    \begin{align*}
        \fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}}M[\nabla_{||}f]^2 d\tau dt dx\lesssim  \fint_Q M[\nabla_{||}f]^2 dx
    \end{align*}

    
    %============================
    
    Let us look at the expression of the nontangential maximal function. Let \(y\in \partial\Omega\) and \(Q\subset\partial\Omega\) a boundary ball with center in \(y\). Let \(\eta_Q\in C_0^\infty(2Q\) be a smooth cut-off function with \(\eta_Q\equiv 1\) on \(Q\) and \(|\nabla \eta_Q|\lesssim 1\), such that \((\eta_{2^kQ\setminus 2^{k-1}Q})_k\) be a partition of unity.
    \begin{align*}
        &\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}f(x)|^2 d\tau dt dx
        \\
        &\sum_{k\geq 2}\fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}(f\chi_{2^kQ\setminus 2^{k-1}Q})(x)|^2 d\tau dt dx
        \\
        &\qquad + \fint_Q\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{\tau^2}{\sqrt{t^2-\tau^2}} |\nabla e^{-\tau^2L^t}(f\chi_{2Q})(x)|^2 d\tau dt dx
        \\
        &\sum_{k\geq 2}\fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{1}{l(Q)^n}\frac{e^{-c\frac{2^{2k}l(Q)^2}{\tau}}}{\sqrt{t^2-\tau^2}} \Vert f\Vert_{L^2(2^kQ\setminus 2^{k-1}Q)}^2 d\tau dt
        \\
        &\qquad + \fint_{l(Q)}^{2l(Q)}\frac{1}{t^2}\int_0^t\frac{1}{l(Q)^n}\frac{1}{\sqrt{t^2-\tau^2}} \Vert f\Vert_{L^2(2Q)}^2 d\tau dt
    \end{align*}


    
    We have by Minkowski inequality, and a dualising function \(\Vert g^t\Vert_{L^2(\mathbb{R}^n)}=1\) for every \(0<t<\infty\)
    \begin{align*}
        \int_{\Omega}\frac{|W_2f(x,t)|^2}{t}dxdt&=\int_0^\infty \frac{1}{t}\int_{\mathbb{R}^n}\Big(\int_0^t 2\tau e^{-(t^2-t^2)L^t}\mathrm{div}(\partial_t A(x,t)\nabla e^{-\tau^2L^t}f)d\tau\Big)^2dxdt
        \\
        &=\int_0^\infty \frac{1}{t}\Big(\int_0^t \Vert 2\tau e^{-(t^2-t^2)L^t}\mathrm{div}(\partial_t A(x,t)\nabla e^{-\tau^2L^t}f)\Vert_{L^2(\mathbb{R}^n)}d\tau\Big)^2dt
        \\
        &=\int_0^\infty \int_0^t \Vert 2\tau e^{-(t^2-t^2)L^t}\mathrm{div}(\partial_t A(x,t)\nabla e^{-\tau^2L^t}f)\Vert_{L^2(\mathbb{R}^n)}^2 dt
        \\
        &=\int_0^\infty \int_0^t 2\tau \partial_t A(x,t)\nabla e^{-\tau^2L^t}f \cdot \nabla e^{-(t^2-t^2)L^t} dx d\tau dt
        \\
        &=\int_0^\infty \frac{1}{t}\Big(\int_0^t \int_{\mathbb{R}^n}2\tau \partial_t A(x,t)\nabla e^{-\tau^2L^t}f \cdot \nabla e^{-(t^2-t^2)L^t}g^t dx d\tau\Big)^2dt
    \end{align*}
\end{proof}

\end{comment}

Now, we can cite the following established square function bounds in [ULM???]
\begin{lemma}
    Let \(f\in C_C(\mathbb{R}^n)\) with \(\mathrm{supp}(f)\subset \Delta\) for a boundary ball \(\Delta\subset\partial\Omega\). Then
    \begin{enumerate}
        \item \(\frac{1}{\sigma(\Delta)}\int_{T(\Delta)}\frac{|W_2f(x,t)|^2}{t}dxdt\lesssim \Vert\nabla_{||}f\Vert_{L^\infty}\lesssim M[M[\nabla_{||}f]^2](x)\)\label{item:LocalSquareBoundW2}
        \item \(\frac{1}{\sigma(\Delta)}\int_{T(\Delta)}\frac{|t\nabla_{||} W_2f(x,t)|^2}{t}dxdt\lesssim \Vert\nabla_{||}f\Vert_{L^\infty}\lesssim M[M[\nabla_{||}f]^2](x)\)\label{item:LocalSquareBoundNablaW2}
    \end{enumerate}
\end{lemma}

\begin{proof}
    For \eqref{item:LocalSquareBoundW2} we use Minkowski inequality and (???? off-diagonal) to obtain

    \begin{align*}
        &\int_{T(\Delta)}\frac{|W_sf|^2}{s}dxds= \int_0^{\infty}\int_{\mathbb{R}^n}\frac{1}{s}\Big|\int_0^{s} \tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)d\tau\Big|^2 dx ds
        \\
        &\leq \int_0^{l(\Delta)}\frac{1}{s}\Big(\int_0^{s} \Vert\tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(\Delta)} d\tau\Big)^2 dx ds
    \end{align*}
    Let us use off-diagonal estimates (???) and smooth cut-off functions such that \(\sum_k\chi_{2^k\Delta\setminus 2^{k-1}\Delta}=1\) (???) to obtain
    \begin{align*}
        &\Vert\tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(\Delta)}
        \\
        &\leq \sum_{k\geq 2}\Vert\tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\chi_{2^k\Delta\setminus 2^{k-1}\Delta}\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(\Delta)}
        \\
        &\qquad + \Vert\tau e^{-(s^2-\tau^2)L_{||}^s}\mathrm{div}(\chi_{2\Delta}\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(\Delta)}
        \\
        &\leq \sum_{k\geq 2}\frac{\tau}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(2^k\Delta\setminus 2^{k-1}\Delta)}
        \\
        &\qquad + \frac{\tau}{\sqrt{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}f)\Vert_{L^2(2\Delta)}
        \\
        &\leq \sum_{k\geq 2}\sum_{m\geq 2}\frac{\tau}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}(\chi_{2^{k+m}\Delta\setminus 2^{k+m-1}\Delta}(f-(f)_{2^k\Delta}))\Vert_{L^2(2^k\Delta\setminus 2^{k-1}\Delta)}
        \\
        & \qquad + \sum_{k\geq 2}\frac{\tau}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}(\chi_{2^{k+1}\Delta}(f-(f)_{2^k\Delta}))\Vert_{L^2(2^k\Delta\setminus 2^{k-1}\Delta)}
        \\
        &\qquad + \sum_{m\geq 3}\frac{\tau}{\sqrt{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}(\chi_{2^m\Delta\setminus 2^{m-1}\Delta}(f-(f)_{4\Delta}))\Vert_{L^2(2\Delta)}
        \\
        &\qquad + \frac{\tau}{\sqrt{s^2-\tau^2}}\Vert\partial_s \AP(x,s)\nabla e^{-\tau^2L_{||}^s}(\chi_{4\Delta}(f-(f)_{4\Delta}))\Vert_{L^2(2\Delta)}
        \\
        &\leq \sum_{k\geq 2}\sum_{m\geq 2}\frac{1}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2} - c\frac{2^{2m}l(\Delta)^2}{\tau^2}}\Vert\partial_s \AP(\cdot,s)\Vert_\infty\Vert(f-(f)_{2^k\Delta})\Vert_{L^2(2^{k+m}\Delta)}
         \\
        & \qquad + \sum_{k\geq 2}\frac{\tau}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2}}\Vert\partial_s \AP(\cdot,s)\Vert_{L^\infty}\Vert\nabla(\chi(f-(f)_{2^k\Delta})))\Vert_{L^2(2^{k+1}\Delta)}
        \\
        &\qquad + \sum_{m\geq 3}\frac{1}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2m}l(\Delta)^2}{\tau^2}}\Vert\partial_s \AP(\cdot,s)\Vert_\infty\Vert(f-(f)_{4\Delta})\Vert_{L^2(2^m\Delta)}
        \\
        &\qquad + \frac{\tau}{\sqrt{s^2-\tau^2}}\Vert\partial_s \AP(\cdot,s)\Vert_\infty\Vert\nabla(\chi(f-(f)_{4\Delta}))\Vert_{L^2(4\Delta)} =I
    \end{align*}

    We notice that
    \begin{align*}
        \Vert f-(f)_{2^k\Delta}\Vert_{L^2(2^{k+m}\Delta)}&\leq \Vert f-(f)_{2^{k+m}\Delta}\Vert_{L^2(2^{k+m}\Delta)} + \sum_{l=1}^m \Vert(f)_{2^{k+l}\Delta}-(f)_{2^{k+l-1}\Delta}\Vert_{L^2(2^{k+m}\Delta)}
        \\
        &\lesssim 2^{(k+m)}l(\Delta)\Vert \nabla_{||}f\Vert_{L^2(2^{k+m}\Delta)} + \sum_{l=1}^m 2^{k+l}l(\Delta)\Vert\nabla_{||}f\Vert_{L^2(2^{k+m}\Delta)}
        \\
        &\lesssim 2^{(k+m)}l(\Delta)\Vert \nabla_{||}f\Vert_{L^2}\lesssim  2^{(k+m)(\frac{n}{2}+1)}l(\Delta)|\Delta|^{1/2}\Vert \nabla_{||}f\Vert_{L^\infty}
    \end{align*}
    and by Poincar\'{e} inequality (???)
    \begin{align*}
        \Vert \nabla(\chi(f-(f)_{2^k\Delta}))\Vert_{L^2(2^{k}\Delta)}&\leq \Vert \nabla_{||}f\Vert_{L^2(2^{k+1}\Delta)} + \frac{1}{2^kl(\Delta)}\Vert f-(f)_{2^k\Delta} \Vert_{L^2(2^{k+1}\Delta)}\lesssim \Vert \nabla_{||}f\Vert_{L^2(2^{k+1}\Delta)}
        \\
        &\lesssim 2^{n(k+1)/2}|\Delta|^{1/2}\Vert \nabla_{||}f\Vert_{\infty}
    \end{align*}
    and hence since \(\tau,\sqrt{s^2-\tau^2}\leq s\leq l(\Delta)\)
    \begin{align*}
        I&=\Vert\partial_s \AP(\cdot,s)\Vert_\infty\Vert\nabla_{||}f\Vert_{L^\infty}|\Delta|^{1/2}\Big(\sum_{k\geq 2}\sum_{m\geq 2}\frac{2^{(k+m)(\frac{n}{2}+1)}l(\Delta)}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2} - c\frac{2^{2m}l(\Delta)^2}{\tau^2}}
         \\
        & \qquad + \sum_{k\geq 2}\frac{\tau 2^{(k+1)\frac{n}{2}}}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2k}l(\Delta)^2}{s^2-\tau^2}} + \sum_{m\geq 3}\frac{2^{(m+1)(\frac{n}{2}+1)}l(\Delta)}{\sqrt{s^2-\tau^2}}e^{-c\frac{2^{2m}l(\Delta)^2}{\tau^2}} + \frac{\tau}{\sqrt{s^2-\tau^2}}\Big)
    \end{align*}
    We consider the sums as Riemann sums of integral. For instance, the second term corresponds to the integral
    \[\int_0^\infty\frac{\tau}{\sqrt{s^2-\tau^2}}x^{\frac{n}{2}-1}e^{-cx^2\frac{l(\Delta)^2}{s^2-\tau^2}}dx,\]
    which after the change of variables \(y=\frac{l(\Delta)^2}{s^2-\tau^2}x\) gives a convergent integral
    \[\frac{\tau\sqrt{s^2-\tau^2}}{l(\Delta)\sqrt{s^2-\tau^2}}\int_0^\infty y^{\frac{n}{2}-1}e^{-y^2}dy\lesssim C.\]
    Similarly, we obtain in total
    \[I\lesssim 1+ \frac{\tau}{\sqrt{s^2-\tau^2}},\]
    whence
    \[\int_0^{l(\Delta)}\frac{1}{s}\Big(\int_0^s \big(1+\frac{\tau}{\sqrt{s^2-\tau^2}}\big)\Vert\partial_s \AP(\cdot,s)\Vert_\infty\Vert\nabla_{||}f\Vert_{L^\infty}|\Delta|^{1/2} d\tau\Big)^2ds\lesssim \Vert\nabla_{||}f\Vert_{L^\infty}^2|\Delta|\int_0^{l(\Delta)} \Vert\partial_s \AP(\cdot,s)\Vert_\infty^2sds\lesssim \Vert\nabla_{||}f\Vert_{L^\infty}^2|\Delta|.\]
    

    For \eqref{item:LocalSquareBoundNablaW2} we have by Cacciopolli type inequality (???)
    \begin{align*}
        \int_{T(\Delta)}\frac{|t\nabla W_2f(x,t)|^2}{t}dxdt&\lesssim \int_{T(2\Delta)}\frac{|W_2f(x,t)|^2}{t}dxdt + |\Delta|\int_0^{2l(\Delta)}\Vert\partial_t A(\cdot,t)\Vert_{L^\infty(\mathbb{R}^n)}^2t\Vert\nabla_{||}f\Vert_{L^\infty(\mathbb{R}^n)}^2dt
        \\
        &\lesssim |\Delta| \Vert \nabla_{||}f\Vert_{L^\infty(\mathbb{R}^n)}
    \end{align*}
\end{proof}


\subsection{The function \(W_1f\)}

\begin{lemma}
    Let \(f\in C_C(\mathbb{R}^n)\) with \(\mathrm{supp}(f)\subset \Delta\) for a boundary ball \(\Delta\subset\partial\Omega\). Then
    \begin{enumerate}
        \item \(\int_{\Omega}\frac{|W_1f(x,t)|^2}{t}dxdt\lesssim \Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}\)\label{item:GlobalSquareBoundW1}
        \item \(\int_{\Omega}\frac{|t\nabla W_1f(x,t)|^2}{t}dxdt\lesssim \Vert M[\nabla_{||}f]\Vert_{L^2(\mathbb{R}^n)}\)\label{item:GlobalSquareBoundNablaW1}
    \end{enumerate}
\end{lemma}

\begin{proof} We start with the proof of \eqref{item:GlobalSquareBoundW1}
\begin{align*}
    \int_\Omega\frac{|tL^te^{-t^2L^t}f|^2}{t}dxdt &\lesssim\int_0^\infty\int_{\mathbb{R}^n}\AP\nabla e^{-t^2 L^t}f(x) \cdot \nabla L^te^{-t^2 L^t}f(x) t dx dt
    \\
    &\qquad =\lesssim\int_0^\infty\frac{1}{t}\Vert\nabla e^{-t^2 L^t}f\Vert_{L^2(\mathbb{R}^n)}^2 +  t^3\Vert\nabla L^te^{-t^2 L^t}f\Vert_{L^2(\mathbb{R}^n)}^2  dx dt
    \\
    &\qquad =\lesssim\int_0^\infty\frac{1}{t}\Vert\nabla e^{-t^2 L^t}f\Vert_{L^2(\mathbb{R}^n)}^2 +  t\Vert\nabla e^{-t^2 L^t}(tL^tf)\Vert_{L^2(\mathbb{R}^n)}^2  dx dt=:I+II.
\end{align*}
First looking at \(I\), we do the following computation with \(g=f\) to handle the second term for a different \(g\) later in the same way. We have
\begin{align*}
t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2(\mathbb{R}^n)}^2&=\int_{\mathbb{R}^n}L^{t}e^{-t^2 L^{t}}g  \cdot e^{-t^2 L^{t}}g t dx
\\
&=\int_{\mathbb{R}^n}\partial_t(e^{-t^2 L^{t}}g) \cdot e^{-t^2 L^t}f dx
\\
&=\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx -\int_{\mathbb{R}^n}\Big(\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}g)d\tau\Big) e^{-t^2 L^t}g dx
\\
&\qquad - 
\int_{\mathbb{R}^n}e^{-t^2L^t}(\partial_tg)\cdot e^{-t^2 L^t}g dx
\\
&=\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx - \int_0^t\int_{\mathbb{R}^n}2\tau \partial_t\AP\nabla e^{-t^2L^t}g\cdot \nabla e^{-(t^2-\tau^2) (L^{t})^*}e^{-t^2 L^t}g dxd\tau
\\
&=\partial_t\Vert e^{-t^2 L^{t}}g\Vert_{L^2}^2 - \int_0^t 2\tau \Vert\partial_t\AP\Vert_\infty\Vert\nabla g\Vert_{L^2}^2 d\tau
\\
&=\partial_t\Vert e^{-t^2 L^{t}}g\Vert_{L^2}^2 - t^2\Vert\partial_t\AP\Vert_\infty\Vert\nabla g\Vert_{L^2}^2 d\tau.
\end{align*}
For the first term we observe
\begin{align*}
    &\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx=\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  \partial_t\int_{W}(e^{-t^2 L^{t}}g)^2 dx
    \\
    &=\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  \partial_t\Big(\int_{W}(e^{-t^2 L^{t}}(g-(g)_W))^2 dx - \int_{W}(e^{-t^2 L^{t}}(g)_W)^2dx +2\int_W e^{-t^2 L^{t}}g \cdot e^{-t^2 L^{t}}(g)_W dx\Big)
    \\
    &=\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  \partial_t\Big(\int_{W}(e^{-t^2 L^{t}}(g-(g)_W))^2 dx +2\int_W e^{-t^2 L^{t}}g \cdot e^{-t^2 L^{t}}(g)_W dx\Big)
    \\
    &=\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  \partial_t\Big(\int_{W}(e^{-t^2 L^{t}}(g-(g)_W))^2 dx +2\int_W e^{-t^2 L^{t}}g \cdot e^{-t^2 L^{t}}((g)_W-g) dx + 2\int_{W}(e^{-t^2 L^{t}}g)^2 dx\Big)
\end{align*}
Since we can hide the last term on the left side, since it is equal to the term in the first line, we obtain
\begin{align*}
    &\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  \partial_t\int_{W}(e^{-t^2 L^{t}}g)^2 dx
    \\
    &=\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}  -\partial_t\Big(\int_{W}(e^{-t^2 L^{t}}(g-(g)_W))^2 dx +2\int_W e^{-t^2 L^{t}}g \cdot e^{-t^2 L^{t}}((g)_W-g) dx\Big)
\end{align*}

Now, using the nonnegativity of the integrand, we can conclude
\begin{align*}
    &\int_0^\infty-\frac{1}{2t^2}\frac{d}{d t}\Vert e^{-t^2 L^{t}}f\Vert_2^2 dt=\lim_{a\to 0} \int_a^\infty -\frac{1}{2t^2}\frac{d}{d t}\Vert e^{-t^2 L^{t}}f\Vert_2^2 dt
    \\
    &\lesssim \lim_{a\to 0} -\frac{1}{2a^2}\int_a^\infty \frac{d}{d t}\Vert e^{-t^2 L^{t}}f\Vert_2^2 dt
    \\
    &\lesssim \lim_{a\to 0} -\frac{1}{2a^2}\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}\int_a^\infty -\frac{d}{d t}\Vert e^{-t^2 L^{t}}(f-(f)_W)\Vert_{L^2(W)}^2 - 2\frac{d}{dt}\Big(\int_W e^{-t^2 L^{t}}g \cdot e^{-t^2 L^{t}}((f)_W-f) dx\Big)dt
    \\
    &=\lim_{a\to0}\frac{1}{2a^2}\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}\Vert e^{-a^2 L^{a}}(f-(f)_W)\Vert_{L^2(W)}^2 + \int_W e^{-a^2 L^{a}}f \cdot e^{-a^2 L^{a}}((f)_W-f) dx 
    \\
    &\lesssim \lim_{a\to0}\frac{1}{2a^2}\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}\Vert e^{-a^2 L^{a}}(f-(f)_W)\Vert_{L^2(W)}^2 +C_\sigma\Vert e^{-a^2 L^{a}}((f)_W-f)\Vert_{L^2(W)}^2 
    \\
    &\hspace{30mm}+  \sigma\Vert e^{-t^2 L^{t}}f\Vert_{L^2(W)}^2
\end{align*}
The sum over the last term \(\sigma\sum_W\Vert e^{-t^2 L^{t}}f\Vert_{L^2(W)}^2\) can be written as \(\sigma\int_a^\infty\frac{d}{dt}\Vert e^{-t^2 L^{t}}f\Vert_{L^2(\mathbb{R}^n)}^2\), whence we can hide it on the left hand side. It remains to bound
\begin{align*}
    &\frac{1}{2a^2}\sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}\Vert e^{-a^2 L^{a}}(f-(f)_W)\Vert_{L^2(W)}^2 +C_\sigma\Vert e^{-a^2 L^{a}}((f)_W-f)\Vert_{L^2(W)}^2
    \\
    &\lesssim \sum_{\substack{W\subset\mathbb{R}^n\textrm{ boundary ball},\\ \textrm{finite overlap, and }l(\Delta)\approx a}}\Vert M[\nabla_{||}f]\Vert_{L^2(W)}^2 +C_\sigma\Vert M[\nabla_{||}f]\Vert_{L^2(W)}^2\lesssim \Vert\nabla_{||}f\Vert_{L^2(\partial\Omega)}^2.
\end{align*}

For the second term, we have similarly to (??? before) and \(g=tL^tf\)
\begin{align*}
t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2(\mathbb{R}^n)}^2&=\int_{\mathbb{R}^n}L^{t}e^{-t^2 L^{t}}g  \cdot e^{-t^2 L^{t}}g t dx
\\
&=\int_{\mathbb{R}^n}\partial_t(e^{-t^2 L^{t}}g) \cdot e^{-t^2 L^t}f dx
\\
&=\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx -\int_{\mathbb{R}^n}\partial_s (e^{-t^2L^s}(sL^sf))|_{s=t} e^{-t^2 L^t}g dx
\\
&=\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx -\int_{\mathbb{R}^n}t\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)\cdot e^{-t^2 L^t}g dx
\\
&\qquad-\int_{\mathbb{R}^n}L^t e^{-t^2L^t}f\cdot e^{-t^2 L^t}g dx
\\
&\qquad- \int_{\mathbb{R}^n}tL^t\Big(\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)d\tau\Big) e^{-t^2 L^t}g dx
\end{align*}

Note that by Cacciopolli type inequality (???)
\begin{align*}
    &\int_{\mathbb{R}^n}tL^t\Big(\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)d\tau\Big) e^{-t^2 L^t}g dx=\int_{\mathbb{R}^n}tA\nabla\Big(\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)d\tau\Big) \nabla e^{-t^2 L^t}g dx
    \\
    &=t\Big\Vert\nabla\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)d\tau\Big\Vert_{L^2}^2 +  \sigma t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2}^2
    \\
    &=\frac{1}{t}\Big\Vert\int_0^t2\tau e^{-(t^2-\tau^2) L^{t}}\mathrm{div}(\partial_t\AP\nabla e^{-t^2L^t}f)d\tau\Big\Vert_{L^2}^2 + t\Vert\partial_t \AP\Vert_\infty^2\Vert \nabla f\Vert_{L^2}^2 +  \sigma t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2}^2
    \\
    &=\frac{1}{t}\Big(\int_0^t2\frac{\tau}{\sqrt{t^2-\tau^2}}\Vert\partial_t\AP\Vert_{\infty}\Vert\nabla f\Vert_{L^2}d\tau\Big)^2 + t\Vert\partial_t \AP\Vert_\infty^2\Vert \nabla f\Vert_{L^2}^2 +  \sigma t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2}^2
    \\
    &=t\Vert\partial_t \AP\Vert_\infty^2\Vert \nabla f\Vert_{L^2}^2 +  \sigma t\Vert\nabla e^{-t^2 L^t}g\Vert_{L^2}^2.
\end{align*}
and hence we can hide the last term on the left hand side and continue with (???)
\begin{align*}
&=\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx -\int_{\mathbb{R}^n}t\partial_t\AP\nabla e^{-t^2L^t}f \cdot \nabla e^{-t^2 L^t}g dx
\\
&\qquad-\int_{\mathbb{R}^n}A\nabla e^{-t^2L^t}f\cdot \nabla e^{-t^2 L^t}g dx + t\Vert\partial_t \AP\Vert_\infty^2\Vert \nabla f\Vert_{L^2}^2 
\\
&\lesssim\partial_t\int_{\mathbb{R}^n}(e^{-t^2 L^{t}}g)^2 dx + t\Vert\partial_t\AP\Vert_{L^\infty}^2\Vert \nabla_{||}f\Vert_{L^2}^2 + \sigma t\Vert\nabla e^{-t^2L^t}f\Vert_{L^2}^2  + t\Vert L^te^{-t^2L^t}f\Vert_{L^2}^2.
\end{align*}
The last term can be hidden on the left side of (???) and the third term can also be hidden on the left side of (???). Then we obtain
\begin{align*}
    \int_0^\infty \Vert\nabla e^{-t^2L^t}g\Vert_{L^2(\mathbb{R}^n)}^2t \lesssim \int_0^\infty \partial_t\nabla e^{-t^2L^t}g\Vert_{L^2(\mathbb{R}^n)}^2 + t\Vert\partial_t\AP\Vert_{L^\infty}^2\Vert \nabla_{||}f\Vert_{L^2}^2 dt.
\end{align*}
Since 
\[\int_0^\infty \partial_t\Vert\nabla e^{-t^2L^t}g\Vert_{L^2(\mathbb{R}^n)}^2 dt=\lim_{a\to 0,b\to\infty}\Vert bL^be^{-b^2L^b}f\Vert_{L^2}^2- \Vert aL^ae^{-a^2L^a}f\Vert_{L^2}^2\lesssim \Vert M[\nabla f]\Vert_{L^2}^2\lesssim \Vert\nabla_{||}f\Vert_{L^2}^2.\]


Part \eqref{item:GlobalSquareBoundNablaW1} follows immediately from \eqref{item:GlobalSquareBoundW1} by observing 
\[\int_\Omega \frac{|t\nabla W_1f(x,t)|^2}{t}dxdt\lesssim \int_\Omega \frac{|W_1f(x,t)|^2}{t}dxdt.\]
from use of the Cacciopolli inequality (???).
\end{proof}












\begin{lemma}
    Let \(f\in C_C(\mathbb{R}^n)\) with \(\mathrm{supp}(f)\subset \Delta\) for a boundary ball \(\Delta\subset\partial\Omega\). Then
    \begin{enumerate}
        \item \(\frac{1}{\sigma(\Delta)}\int_{T(\Delta)}\frac{|W_1f(x,t)|^2}{t}dxdt\lesssim \fint_\Delta |\nabla_{||}f|^2 d\sigma\lesssim M[M[\nabla_{||}f]^2](x)\)\label{item:LocalSquareBoundW1}
        \item \(\frac{1}{\sigma(\Delta)}\int_{T(\Delta)}\frac{|t\nabla_{||} W_1f(x,t)|^2}{t}dxdt\lesssim \fint_\Delta |\nabla_{||}f|^2 d\sigma\lesssim M[M[\nabla_{||}f]^2](x)\)\label{item:LocalSquareBoundNablaW1}
    \end{enumerate}
\end{lemma}

\begin{proof}
    First for \eqref{item:LocalSquareBoundW1}. We introduce a smooth cut-off function \(\eta\in C_0^\infty(3\Delta)\) with \(\eta\equiv 1\) on \(2\Delta\) and \(|\nabla \eta|\lesssim \frac{1}{l(\Delta)}\). We obtain

    \begin{align*}
        \int_{T(\Delta)}\frac{|W_1f(x,t)|^2}{t}dxdt=\int_{T(\Delta)}\frac{|W_1(f-(f)_{3\Delta})(x,t)|^2}{t}dxdt\leq \int_{T(\Delta)}\frac{|W_1((f-(f)_{3\Delta})\eta)(x,t)|^2}{t}dxdt + \int_{T(\Delta)}\frac{|W_1((f-(f)_{3\Delta})(1-\eta))(x,t)|^2}{t}dxdt.
    \end{align*}
    Since the first integral is bounded by \(\Vert\nabla( (f-(f)_{3\Delta})\eta)\Vert_{L^2(\mathbb{R}^n)}\lesssim \frac{1}{l(\Delta)}\Vert (f-(f)_{3\Delta}) \Vert_{L^2(3\Delta)} + \Vert \nabla_{||} f\Vert_{L^2(3\Delta)}\lesssim \Vert \nabla_{||} f\Vert_{L^2(3\Delta)}\) by Lemma (??? global bounds) and Poincar\'{e}'s inequality, we only need to deal with the second integral.
    
    We have for a fixed \(t\in (0,l(\Delta))\) with off-diagonal estimates (???) for \(W_1g(x,t)=t\partial_\tau e^{-\tau L^s}g(x)|_{s=t, \tau=t^2}\)

    \begin{align*}
        &\Vert W_1 ((f-(f)_{3\Delta})(1-\eta))\Vert_{L^2(\Delta)}\lesssim \Vert W_1 (\chi_{4\Delta}(f-(f)_{3\Delta})(1-\eta))\Vert_{L^2(\Delta)} +\sum_{k\geq 2}\Vert W_1 (\chi_{2^{k+1}\Delta\setminus 2^{k}\Delta}(f-(f)_{3\Delta}))\Vert_{L^2(\Delta)}
        \\
        &\lesssim \frac{1}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert f-(f)_{3\Delta} \Vert_{L^2(4\Delta\setminus 2\Delta)} + \sum_{k\geq 2}\frac{1}{t}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Vert f-(f)_{3\Delta}\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)}
        \\
        &\lesssim \frac{1}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert f-(f)_{4\Delta} \Vert_{L^2(4\Delta\setminus 2\Delta)} + \frac{1}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert (f)_{4\Delta}-(f)_{3\Delta} \Vert_{L^2(4\Delta\setminus 2\Delta)}
        \\
        &\qquad +\sum_{k\geq 2}\frac{1}{t}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big(\Vert f-(f)_{2^{k+1}\Delta}\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)} + \sum_{j=2}^{k-1} \Vert (f)_{2^{j+1}\Delta}-(f)_{2^j\Delta}\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)} + \Vert (f)_{4\Delta}-(f)_{3\Delta}\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)}\Big)
        \\
        &\lesssim \frac{l(\Delta)}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert \nabla_{||}f \Vert_{L^2(4\Delta\setminus 2\Delta)} + \frac{l(\Delta)}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert\nabla_{||}f \Vert_{L^2(4\Delta\setminus 2\Delta)}
        \\
        &\qquad +\sum_{k\geq 2}\frac{1}{t}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big(2^{k+1}l(\Delta)\Vert \nabla_{||}f\Vert_{L^2(2^{k+1}\Delta)} + \sum_{j=2}^{k-1} 2^{j+1}l(\Delta)\big\Vert \Vert \nabla_{||} f\Vert_{L^2(2^{j+1}\Delta)}\big\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)} + l(\Delta)\big\Vert \Vert \nabla_{||} f\Vert_{L^2(4\Delta)}\big\Vert_{L^2(2^{k+1}\Delta\setminus 2^k\Delta)}\Big)
        \\
        &\lesssim \frac{l(\Delta)^{\frac{n}{2}+1}}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert \nabla_{||}f \Vert_{\infty} + \frac{l(\Delta)^{\frac{n}{2}+1}}{t}e^{-c\frac{l(\Delta)^2}{t^2}}\Vert\nabla_{||}f \Vert_{\infty}
        \\
        &\qquad +\sum_{k\geq 2}\frac{1}{t}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big(2^{(k+1)(\frac{n}{2}+1)}l(\Delta)^{\frac{n}{2}+2}\Vert \nabla_{||}f\Vert_{\infty} + \sum_{j=2}^{k-1} 2^{(k+1)(\frac{n}{2}) + j+1}l(\Delta)^{(j+1)(\frac{n}{2}+1)}\Vert \nabla_{||} f\Vert_{\infty} + l(\Delta)^{\frac{n}{2}+2} \Vert \nabla_{||} f\Vert_{\infty}\Big)
        \\
        &\lesssim \frac{l(\Delta)^{\frac{n}{2}+1}}{t}\Big(e^{-c\frac{l(\Delta)^2}{t^2}} + \sum_{k\geq 2} (k+1)2^{(k+1)(\frac{n}{2}+1)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big)\Vert \nabla_{||} f\Vert_{\infty}
        \\
        &\lesssim \frac{l(\Delta)^{\frac{n}{2}+1}}{t}\Big(\sum_{k\geq 1} (k+1)2^{(k+1)(\frac{n}{2}+1)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big)\Vert \nabla_{||} f\Vert_{\infty}
        \\
        &\lesssim \frac{l(\Delta)^{\frac{n}{2}+1}}{t}\Big(\sum_{k\geq 1} 2^{(k+1)(\frac{n}{2}+2)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big)\Vert \nabla_{||} f\Vert_{\infty}
    \end{align*}

    With this in hand, we return now to 
    \begin{align*}
    \int_{T(\Delta)}\frac{|W_1((f-(f)_{3\Delta})(1-\eta))(x,t)|^2}{t}dxdt&\lesssim \int_0^{l(\Delta)}\frac{l(\Delta)^{n+2}}{t^3}\Big(\sum_{k\geq 1} 2^{(k+1)(\frac{n}{2}+2)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big)^2\Vert \nabla_{||} f\Vert_{\infty}^2dt
    \\
    & \lesssim l(\Delta)^{n+2}\Vert \nabla_{||} f\Vert_{\infty}^2\int_0^{l(\Delta)}\Big(\sum_{k\geq 1} \frac{1}{t^{3/2}}2^{(k+1)(\frac{n}{2}+2)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\Big)^2dt
    \end{align*}

    We can study the function\(t\mapsto \frac{1}{t^{3/2}}e^{-c\frac{a^2}{t^2}}\) for \(t\in (0,l(\Delta))\) and observe that it attains its maximum if \(t=l(\Delta)\), whence
    \[\sum_{k\geq 1} \frac{1}{t^{3/2}}2^{(k+1)(\frac{n}{2}+2)}e^{-c\frac{2^{2k}l(\Delta)^2}{t^2}}\lesssim \frac{1}{l(\Delta)^{3/2}}\sum_{k\geq 1} 2^{(k+1)(\frac{n}{2}+2)}e^{-c2^{2k}}\]
    Similarly to (???), we consider the sum as Riemann sums of the corresponding integral
    \[\int_0^\infty x^{\frac{n}{2}+1}e^{-cx^2}dx,\]
    which converges. Hence we obtain in total
    
    \begin{align*}
    \int_{T(\Delta)}\frac{|W_1((f-(f)_{3\Delta})(1-\eta))(x,t)|^2}{t}dxdt& \lesssim l(\Delta)^{n+2}\Vert \nabla_{||} f\Vert_{\infty}^2\int_0^{l(\Delta)}\frac{1}{l(\Delta)^3}dt= \Vert \nabla_{||} f\Vert_{\infty}^2.
    \end{align*}
\end{proof}
